Total Variation Floodgate for Variable Importance Inference in Classification

Inferring variable importance is the key problem of many scientific studies, where researchers seek to learn the effect of a feature $X$ on the outcome $Y$ in the presence of confounding variables $Z$. Focusing on classification problems, we define the expected total variation (ETV), which is an intuitive and deterministic measure of variable importance that does not rely on any model context. We then introduce algorithms for statistical inference on the ETV under design-based/model-X assumptions. These algorithms build on the floodgate notion for regression problems (Zhang and Janson 2020). The algorithms we introduce can leverage any user-specified regression function and produce asymptotic lower confidence bounds for the ETV. We show the effectiveness of our algorithms with simulations and a case study in conjoint analysis on the US general election.

==> discussion/comparison.tex <==
\section{A power comparison of the conditional randomization tests}
%\subsection{Conditional randomization test}




% \subsection{Comparison}
% In this section, let $X_i\simiid\mathcal N(0,1)$, $g$ be the logit function, $\theta_1$ be the alternative, and $\hat\theta$ be the unconstrained MLE. Consider the following tests.

% \begin{center}
% \begin{tabular}{ |c|c|c|c| } 
%  \hline
%   & Model-X & Traditional \\ 
%  \hline
% Two-sided & when $|\sqrt n\overline{ZX}|\ge z_{\alpha/2}$ & when $2\log\frac{\ell(\hat\theta)}{\ell(0)}>\chi_{1,\alpha}^2$  \\ 
%  \hline
%  One-sided & when $\sqrt n\overline{ZX}\ge z_{\alpha}$ & when $2\log\frac{\ell(\max(0,\hat\theta))}{\ell(0)}>\chi_{1,2\alpha}^2$ \\ 
%  \hline
%  Simple & when $\frac{\ell(\theta_1)}{\ell(0)}$ is large, cutoff conditional on $Z$ & when $\frac{\ell(\theta_1)}{\ell(0)}$ is large, cutoff conditional on $X$ \\ 
%  \hline
% \end{tabular}
% \end{center}

% In the simulations, we find
% \begin{itemize}
%     \item for small (5) or moderate (10, 15) $n$, the asymptotic tests are not valid (one-sided and two-sided generalized LRT);
%     \item among the four valid tests, the simple model-X test is (provably) the most powerful test;
%     \item the one-sided model-X test is (provably and obviously) more powerful than the two-sided model-X test;
%     \item when the signal strength is weak or moderate ($\le0.8$), the one-sided model-X test has minimal power loss compared to the simple model-X test;
%     \item when the sample size is small ($n=5$), the one-sided model-X test has comparable power with the simple model-Y test;
%     \item when the sample size is moderate ($n=10$), the simple model-Y test has similar power with the simple model-X test, a fact which agrees with \citet{lehmann2006testing}.
% \end{itemize} 
% \begin{figure}
%     \centering
% \includegraphics[width = \textwidth]{figures/logistic5.pdf}
%     \caption{Comparision of different tests with $n=5$.} 
%     \label{figure:log5}
% \end{figure}
% \begin{figure}
%     \centering
% \includegraphics[width = \textwidth]{figures/logistic10.pdf}
%     \caption{Comparision of different tests with $n=10$.} 
%     \label{figure:log10}
% \end{figure}

% \begin{figure}
%     \centering
% \includegraphics[width = \textwidth]{figures/logistic15.pdf}
%     \caption{Comparision of different tests with $n=15$.} 
%     \label{figure:log15}
% \end{figure}

% \begin{figure}
%     \centering
% \includegraphics[width = \textwidth]{figures/logistic100.pdf}
%     \caption{Comparision of different tests with $n=100$.} 
%     \label{figure:log100}
% \end{figure}





==> discussion/elliptical.tex <==
\section{Knockoffs for elliptical distributions}

\ejc{I don't understand how this fits into the rest of the paper. I am worried that this would get lost.}

\label{sec:knockell}
\subsection{Elliptical distributions}
\begin{defi}
A real random vector $\bm X$ is said to have an elliptical distribution with median $\bm\mu$, if the characterisitic function of $\bm X-\bm\mu$ admits the form
\begin{equation*}
\varphi_{\bm X-\bm\mu}(\bm t)=\psi(\bm t\bm\Sigma\bm t^\top),
\end{equation*}
where $\psi$ is a scalar function, and $\bm\Sigma$ is nonnegative-definite. We denote it as $\bm X\sim\mathcal E(\bm\mu,\bm\Sigma,\psi)$.
\end{defi}
If $\bm X$ has finite second moment, then
\begin{equation*}
\Cov(\bm X)=-\varphi_{\bm X-\bm\mu}''(\bm0)=-2\psi'(0)\cdot\bm\Sigma.
\end{equation*}
Hence, $\bm\Sigma$ is proportional to the covariance matrix.

%It's obvious from the definition that if $X$ has an elliptical distribution, then any subvector of $X$ has an elliptical distribution as well.
%In cases where this subvector is in the same parametric family as the full vector, we can use it as a way to construct knockoffs.
We now introduce the general stochastic representation of elliptical distributions given in \citet{cambanis1981theory} and \citet{frahm2004generalized}, which will be very useful in our proposed method for knockoff construction.

\begin{thm}
(Theorem 1 in \citet{cambanis1981theory}) $\bm X\sim\mathcal E(\bm\mu,\bm\Sigma,\psi)$ with $\rank(\bm\Sigma)=k$ if and only if
\begin{equation*}
\bm X^\top=\bm\mu^\top+R\bm\Lambda\bm U^{(k)},
\end{equation*}
where $\rank(\bm\Lambda_{d\times k}=k)$, $\bm\Lambda\bm\Lambda^\top=\bm\Sigma$, $\bm U^{(k)}\sim\Unif(\mathcal S^{k-1})$, $R$ is a non-negative random variable independent of $\bm U^{(k)}$, and $\psi(u)=\e(\Omega_k(R^2u))$, where $\Omega_k(\|\bm t\|^2)=\varphi_{\bm U^{(k)}}(\bm t)$ is the characteristic function of $\bm U^{(k)}$.
\end{thm}

A knockoff construction for $\bm X\sim\mathcal E(\bm\mu,\bm\Sigma,\psi)$ can be done if we can find a $\bXk$ defined on the same (augmented) probability space such that $(\bm X,\bXk)$ is also an elliptical random vector with the matrix parameter having the corresponding form \eqref{eq:knockoff-cov}. When this is possible, $\bXk$ is naturally a knockoff for $\bm X$, so we can sample our knockoff for $\bm X$ from $\bXk\mid \bm X$ (see Appendix \ref{subapp:cond-ell-dist}). For this to be possible, $\bm X$ is ``almost certain'' to be related to the normal distribution; see Appendix \ref{subapp:gaussian-special}.

We present the multivariate $t$-distribution and the multivariate Laplace distribution as examples in Appendix \ref{subapp:elliptical}. In practice, after one estimates the mean and covariance, it might make more sense to check the empirical distribution of $(\bm X-\bm\mu)\bm\Sigma^{-1}(\bm X-\bm\mu)^\top$ and pick a corresponding elliptical distribution, instead of using Gaussian directly
%\cite{sesia2018gene}
. It should be noted that the generating variable can be discrete, resulting in a discrete mixture of Gaussian components. It has been noticed that some data require carefully treatment regarding their tail behavior. For example, it is pointed out in \citet{kotz2004multivariate} that the multivariate $t$-distribution is better suited to model market returns than Gaussian. To the best of our knowledge, this is the first result on high-dimensional variable selection when the covariates are allowed to have heavy tails, where traditional methods are not guaranteed to work \citep{javanmard2014confidence}.

%\subsubsection{Meta-elliptical distributions}
%{\color{red} WW: this section can be deleted}{\color{blue} [SB: I think we should keep statement of the fact that knockoffs are preserved under coordinate transformations. This is a useful fact for practitioners, and worth including in the Appendix. We can defer these two definitions to the supplementary material, however.]}
Using copulas, we can generalize knockoff construction to some meta-elliptical distributions. See Appendix \ref{subapp:meta-details} for details. More generally, the pairwise exchangeability is always preserved under coordinate transformations.

\subsection{Proofs of Appendix \ref{app:knockell}}
\begin{proof}[Proof of Theorem \ref{theorem:beta}]
We only consider the case $m>p$ because the alternative case is not helpful for constructing knockoffs. Let such $\bm Z$ have representation
\begin{equation*}
\bm Z^\top=(\bm\mu^*)^\top+T\bm\Lambda^*\bm U^{(m)},
\end{equation*}
where
\begin{equation*}
\bm\Lambda^*=\left[
  \begin{array}{cc}
\bm\Lambda_{11} & 0\\
\bm\Lambda_{21} & \bm\Lambda_{22}\\
  \end{array}
\right], \bm\Lambda_{11}\bm\Lambda_{11}^\top=\bm\Sigma.
\end{equation*}
This implies
\begin{equation*}
\bm X\eqd\bm Z_{1:p}=\bm\mu^*_{1:p}+(T\cdot\sqrt V)\left(\bm\Lambda_{11}\bm U^{(p)}\right)^\top,
\end{equation*}
where $T$, $V$ and $\bm U^{(p)}$ are mutually independent, and $V\eqd\|\bm U_{1:p}^{(m)}\|^2\sim\Be(\frac p2,\frac m2-\frac p2)$.

By a comparison of the median, we have $\bm\mu=\bm\mu^*_{1:p}$. Recall that $\bm\Lambda\bm\Lambda^\top=\bm\Lambda_{11}\bm\Lambda_{11}^\top=\bm\Sigma$. Thus,
\begin{equation*}
R^2=(\bm X-\bm\mu)\bm\Sigma^{-1}(\bm X-\bm\mu)^\top\eqd(\bm Z_{1:p}-\bm\mu^*_{1:p})\bm\Sigma^{-1}(\bm Z_{1:p}-\bm\mu^*_{1:p})^\top=T^2V.
\end{equation*}
Since we are dealing with non-negative random variables, this translates to
%\begin{equation}
$R\eqd T\cdot\sqrt V$.
%\end{equation}
\end{proof}

\begin{proof}[Proof of Theorem \ref{theorem:ell-gaussian}]
The condition is equivalent to that for each $n>p$, there exists an $n$-dimensional elliptical random vector $\bm Z^{(n)}$, such that $\bm Z^{(n)}_{1:p}\eqd\bm X$. This is due to the fact that any sub-vector of a full-rank elliptical random vector is also a full-rank elliptical random vector. By Theorem \ref{theorem:beta}, we have representations
\begin{equation*}
R\eqd R_n\cdot\sqrt{V_n}, R_n\ci V_n, n>p.
\end{equation*}
where $V_n\eqd\|\bm U^{(n)}_{1:p}\|^2\sim\Be(p/2,n/2-p/2)$.

Thus, for any $n>p$, we can represent $R^2$ as the product of a $\Be(p/2,n/2-p/2)$ random variable $V_n$ and another independent random variable $R_n^2$. Without loss of generality, assume $R>0$ almost surely. We would then have
\begin{equation*}
2\log R\eqd2\log R_n+\log V_n,2\log R_n\ci\log V_n,n>p.
\end{equation*}
Let $\varphi$ and $\varphi_n$ be the characteristic functions of $2\log R$ and $2\log R_n$, and we will get equivalently,
\begin{equation*}
\varphi(t)=\varphi_n(t)\frac{\Gamma(\frac p2+it)\Gamma(\frac n2)}{\Gamma(\frac p2)\Gamma(\frac n2+it)},n>p.
\end{equation*}
Consider the random variable $2\log R_n-\log\frac n2$. Its characteristic function is
\begin{equation*}
\varphi_n^*(t)=\e(e^{i2t\log R_n}e^{-it\log\frac n2})=\varphi_n(t)/(\frac n2)^{it}.
\end{equation*}
Note that
\begin{equation*}
\varphi_n^*(t)=\varphi_n(t)/(\frac n2)^{it}=\varphi(t)\frac{\Gamma(\frac p2)\Gamma(\frac n2+it)}{\Gamma(\frac p2+it)\Gamma(\frac n2)}\frac{1}{(\frac n2)^{it}},
\end{equation*}
and
\begin{equation*}
\varphi^*(t)=\lim_{n\to\infty}\varphi_n^*(t)=\varphi(t)\frac{\Gamma(\frac p2)}{\Gamma(\frac p2+it)}\lim_{n\to\infty}\frac{\Gamma(\frac n2+it)}{\Gamma(\frac n2)(\frac n2)^{it}}=\varphi(t)\frac{\Gamma(\frac p2)}{\Gamma(\frac p2+it)}, \forall t\in\rr.
\end{equation*}
Since $\varphi^*(t)$ is obviously continuous at $t=0$, by L\'evy's continuity theorem, $\varphi^*(t)$ is the characteristic function of some random variable $R^*$. Since
\begin{equation*}
\varphi(t)=\frac{\varphi^*(t)}{2^{it}}\frac{2^{it}\Gamma(\frac p2+it)}{\Gamma(\frac p2)},
\end{equation*}
and $\frac{\varphi^*(t)}{2^{it}}$ is the characteristic function of $R^*-\log2$, and $\frac{2^{it}\Gamma(\frac p2+it)}{\Gamma(\frac p2)}$ is the characteristic function of $\log(\chi_p^2)$, we have
\begin{equation*}
2\log R\eqd R^*-\log 2+\log V, V\sim\chi_p^2, R^*\ci V.
\end{equation*}
Let $T=e^{\frac{R^*-\log 2}{2}}$, we have $R\eqd T\cdot\sqrt{V}$, $V\sim\chi_p^2$ and $T\ci V$.
\end{proof}



\section{Details of elliptical knockoffs}
\subsection{Conditional elliptical distributions}
\label{subapp:cond-ell-dist}
\begin{thm}
(Theorem 7 in \citet{frahm2004generalized}) Let $\bm X\sim\mathcal E(\bm\mu,\bm\Sigma,\psi)$ with $\bm\mu=(\bm\mu_1,\bm\mu_2)\in\rr^{k+(d-k)}$ and $\rank(\bm\Sigma)=r$.
Let
\begin{equation*}
\bm C=\left[
  \begin{array}{cc}
\bm C_{11} & 0\\
\bm C_{21} & \bm C_{22}\\
  \end{array}
\right]\in\rr^{d\times r}
\end{equation*}
be the generalized Cholesky root of $\bm\Sigma$, where $\bm C_{11}\in\rr^{k\times k}$, $\bm C_{21}\in\rr^{(d-k)\times k}$ and $\bm C_{22}\in\rr^{(d-k)\times(r-k)}$. The conditional distribution $\bm X_2 \mid \bm X_1$, if it exists, is also elliptical with representation
\begin{equation*}
\bm X_2 \mid \bm X_1=\bm x_1\eqd\bm\mu^*+R^*\bm \left(\bm C_{22}\bm U^{(r-k)}\right)^\top,
\end{equation*}
where
\begin{equation*}
R^*\sim R\sqrt{1-\beta} \mid  R\sqrt\beta\bm U^{(k)}=\bm C_{11}^{-1}(\bm x_1-\bm\mu_1)^\top,
\end{equation*}
\begin{equation*}
(\bm\mu^*)^\top=\bm\mu_2^\top+\bm C_{21}\bm C_{11}^{-1}(\bm x_1-\bm\mu_1)^\top,
\end{equation*}
$\bm U^{(k)}\sim\Unif(\mathcal S^{k-1})$, $\bm U^{(r-k)}\sim\Unif(\mathcal S^{r-k-1})$, $\beta\sim\Be(\frac k2,\frac{d-k}2)$ and $R$, $\beta$, $\bm U^{(k)}$ and $\bm U^{(r-k)}$ are independent.
\end{thm}

\subsection{Why are Gaussian distributions special?}
\label{subapp:gaussian-special}
\begin{thm}
\label{theorem:beta}
Let ${\bm X}\sim\mathcal E(\bm\mu,\bm\Sigma,\psi)$ be a $p$-dimensional elliptical random vector, where $\rank(\bm\Sigma)=p$. There is an $n$-dimensional elliptical random vector $\bm Z\sim\mathcal E(\bm\mu^*,\bm\Sigma^*,\psi^*)$, where $\rank(\bm\Sigma^*)=m>p$, such that $\bm Z_{1:p}\eqd {\bm X}$, if and only if in the representation
\begin{equation*}
{\bm X}^\top=\bm\mu^\top+R\bm\Lambda\bm U^{(p)},
\end{equation*}
$R$ can be written as $T\cdot\sqrt{V}$, $V\sim\Be(\frac p2,\frac m2-\frac p2)$, independent of $T$.
\end{thm}



\begin{thm}
\label{theorem:ell-gaussian}
Let ${\bm X}\sim\mathcal E(\bm\mu,\bm\Sigma,\psi)$ be a $p$-dimensional elliptical random vector, where $\rank(\bm\Sigma)=p$. If there are infinitely many $n$'s greater than $p$, for which there is an $n$-dimensional full-rank elliptical random vector $\bm Z$, such that $\bm Z_{1:p}\eqd {\bm X}$, then in the representation
\begin{equation*}
{\bm X}^\top=\bm\mu^\top+R\bm\Lambda\bm U^{(p)},
\end{equation*}
$R$ can be written as $T\cdot\sqrt{V}$, $V\sim\chi^2_{p}$, independent of $T$. Note that $\sqrt{V}\bm U^{(p)}\sim\mathcal N(\bm0,\bm I_p)$, so $\bm X^\top\eqd\bm\mu^\top+T\bm\Lambda\bm Z^\top$, where $\bm Z\sim\mathcal N(\bm0,\bm I_p)$, independent of $T$. The converse is obviously also true.
\end{thm}

Theorem \ref{theorem:ell-gaussian} shows that if we want to sample knockoffs for a family of elliptical distributions of any dimension by embedding it into another elliptical random vector twice the length, then this family of elliptical distributions necessarily can be written as the product of a multivariate Gaussian random vector and another independent random variable. It should be noted that there do exist random variables supported on $(0,\infty)$ that cannot be written as a product of $\chi_p^2$ and another independent distribution (e.g., $\chi_q^2$, $q>p$).%If $X\sim\chi_q^2$, $q>p$, can be written as the product of independent random variables $Y\sim\chi_p^2$ and $Z$, then $\log X\sim\log Y+\log Z$ (obviously, $Z>0$, $a.s.$). This implies $\Var(\log X)\ge\Var(\log Y)$ (due to their existence). However,
%Let $\varphi_X$ and $\varphi_Y$ be the charactersitic functions of $\log X$ and $\log Y$, and we have $\varphi_X/\varphi_Y$ is a valid characteristic function.
%since we know $Y$ can be written as the product of $X$ and another independent $\Be(p/2,q/2-p/2)$, we have $\Var(\log Y)>\Var(\log X)$, which is a contradiction.
%$\varphi_Y/\varphi_X$ is a valid characteristic function. However, if a function and its reciprocal are both valid characteristic functions, its absolute value will always be one. Let $W_1$ and $W_2$ be two independent random variables with this characteristic function, then the characteristic function of $W_1-W_2$ will be constant $1$, which means $W_1-W_2=0$, $a.s.$, so $W_1$ and $W_2$ are constants almost surely. However, this is not the case in the example above, hence a contradiction. An easier way to check this is if $X$ and be written as the product of $Y$ and another independent random variable, $\Var(\log X)$ should be greater than $\Var(\log Y)$ (when they exist).

\subsection{Meta-elliptical distributions}
\label{subapp:meta-details}
We introduce meta-elliptical distributions, and show how knockoffs can be constructed for this class of distributions.
\begin{defi}
Let ${\bm X}=(X_1,X_2,\dots,X_p)$ be a random vector with continuous marginal cumulative distribution functions $F_j$, $1\le j\le p$. The copula of ${\bm X}$ is defined to be the joint cumulative distribution function of $(F_1(X_1),F_2(X_2),\dots,F_p(X_p))$, i.e.,
\begin{equation*}
C_{\bm X}(u_1,u_2,\dots,u_p)=\p(F_1(X_1)\le u_1,F_2(X_2)\le u_2,\dots,F_p(X_p)\le u_p),\bm u\in[0,1]^p.
\end{equation*}
\end{defi}

\begin{defi}
(Definition 8 in \citet{frahm2004generalized})
Let ${\bm X}=(X_1,X_2,\dots,X_p)$ be a random vector with marginal cumulative distribution functions $F_j$, $1\le j\le p$. ${\bm X}$ is said to be meta-elliptically distributed, if
\begin{equation*}
\p(F_1(X_1)\le u_1,F_2(X_2)\le u_2,\dots,F_p(X_p)\le u_p)=C_{\bm Z}(u_1,u_2,\dots,u_p),u\in[0,1]^p,
\end{equation*}
where $C_{\bm Z}$ is the copula of $\bm Z\sim\mathcal E(\bm\mu,\bm\Sigma,\psi)$. This is denoted as ${\bm X}\sim\mathcal M\mathcal E(\bm\mu,\bm\Sigma,\psi)$.
\end{defi}
Since ${\bm X}\sim\mathcal M\mathcal E(\bm\mu,\bm\Sigma,\psi)$ admits representation $X_j=F_j^{-1}(G_j(Y_j))$, $1\le j\le p$, where $F_j$ and $G_j$ are cumulative distribution functions of $X_j$ and $Y_j$, we can easily generate knockoffs for ${\bm X}$ if we can do so for $\bm Z$. Of course, the same method applies to other coordinate-wise transformations.

%As pointed out in \citet{whitt1976bivariate}, we can match all pairwise correlations this way.

\subsection{Elliptical knockoffs: examples}
\label{subapp:elliptical}
\subsubsection{Multivariate \texorpdfstring{$t$}{t}-distribution}
\begin{defi}
If $\bm Z\sim\mathcal N(\bm0, \bm\Sigma)$ and $U\sim\chi_\nu^2$ are indenpendent, ${\bm X}=\bm\mu+\frac{\bm Z}{\sqrt{U/\nu}}$ is said to have the multivariate-$t$ distribution $t_\nu(\bm\mu,\bm\Sigma)$.
\end{defi}

The characteristic function of ${\bm X}-\mu$ is
\begin{equation*}
\begin{aligned}
\varphi_{{\bm X}-\bm\mu}(\bm t)&=\e(\exp(i\bm t\frac{\bm Z^\top}{\sqrt{U/\nu}}))=\e(\e(\exp(i\bm t\frac{\bm Z^\top}{\sqrt{U/\nu}}) \mid  U))\\
&=\e(\exp(-\frac12(\frac{\bm t}{\sqrt{U/\nu}})\bm\Sigma(\frac{\bm t}{\sqrt{U/\nu}})^\top))=\e(\exp(-\frac{\nu}{2U}\bm t\bm\Sigma\bm t^\top)),
\end{aligned}
\end{equation*}
which is a function of $\bm t\bm\Sigma\bm t^\top$. By definition, $t_\nu(\bm\mu,\bm\Sigma)$ is an elliptical distribution.

Let
\begin{equation*}
(\bm X,\bXk)\sim t_\nu((\bm\mu,\bm\mu),\bm\Gamma=\left[
  \begin{array}{cc}
\bm\Sigma & \bm\Sigma-\diag(\bm s)\\
\bm\Sigma-\diag(\bm s) & \bm\Sigma\\
  \end{array}
\right])
\end{equation*}
It then admits representation
\begin{equation*}
(\bm X,\bXk)=(\bm\mu,\bm\mu)+\frac{1}{\sqrt{U/\nu}}(\bm Z,\tilde{\bm Z}), (\bm Z,\tilde{\bm Z})\sim\mathcal N(\bm0,\bm\Gamma), U\sim\chi_\nu^2\text{ independently}.
\end{equation*}
Pairwise exchangeablity of $(\bm Z,\tilde{\bm Z})$ implies pairwise exchangeablity of $({\bm X},\bXk)$. Thus, $\bXk$ is knockoff for ${\bm X}$, and ${\bm X}\sim t_\nu(\bm\mu,\bm\Sigma)$! In practice, Sampling from $\bXk \mid  {\bm X}$ can be easily implemented by first sampling $U \mid  {\bm X}\sim\Ga(\nu+p,\frac12+\frac{({\bm X}-\bm\mu)\bm\Sigma^{-1}({\bm X}-\bm\mu)^\top}{2\nu})$, where the second parameter is the rate parameter. Then, we sample from $\bXk\mid U,\bm X$, which is a multivariate normal distribution. In fact,
\begin{equation*}
\bXk\mid  {\bm X}\sim t_{\nu+p}({\bm X}-({\bm X}-\bm\mu)\bm\Sigma^{-1}\diag(\bm s),\frac{\nu+({\bm X}-\bm\mu)\bm\Sigma^{-1}({\bm X}-\bm\mu)^\top}{\nu+k}(2\diag(\bm s)-\diag(\bm s)\bm\Sigma^{-1}\diag(\bm s))).
\end{equation*}

Note that a zero in the covariance matrix doesn't imply independence in the multivariate-$t$ distribution, and other non-Gaussian elliptical distributions in general. Hence, if such independence structure is available, one should model them separately to reflect that knowledge, and not model them jointly. It has also been pointed out that the uncorrelated multivariate $t$-distribution captures the heavy tail better than independent $t$ distributions \citep{kelejian1985independent}.

\subsubsection{Multivariate Laplace distribution}
\begin{defi}
A symmetric multivariate Laplace distribution with mean $\bm\mu$ and covariance matrix $\bm\Sigma$, denoted by $\Laplace(\bm\mu,\bm\Sigma)$, is the distribution with characterisitic function
\begin{equation*}
\varphi(\bm t)=\frac{\exp(i\bm\mu\bm t^\top)}{1+\frac12\bm t\bm\Sigma\bm t^\top}.
\end{equation*}
\end{defi}

If ${\bm X}\sim\Laplace(\bm\mu,\bm\Sigma)$,
\begin{equation*}
\varphi_{{\bm X}-\bm\mu}(\bm t)=\varphi(\bm t)/\exp(i\bm\mu\bm t^\top)=\frac{1}{1+\frac12\bm t\bm\Sigma\bm t^\top},
\end{equation*}
which is a function of $\bm t\bm\Sigma\bm t^\top$. This makes it an elliptical distribution.

Note that if
\begin{equation*}
(\bm X,\bXk)\sim\Laplace((\bm\mu,\bm\mu),\bm\Gamma=\left[
  \begin{array}{cc}
\bm\Sigma & \bm\Sigma-\diag(\bm s)\\
\bm\Sigma-\diag(\bm s) & \bm\Sigma\\
  \end{array}
\right]),
\end{equation*}
${\bm X}$ and $\bXk$ are knockoff copies of each other, since the characteristic function is symmetric in every pair.
The characteristic function of ${\bm X}$ is
\begin{equation*}
\varphi_{\bm X}(\bm t)=\varphi_\text{joint}((\bm t,\bm0))=\frac{\exp(i(\bm\mu, \bm\mu)\left(
  \begin{array}{c}
\bm t^\top\\
\bm0^\top\\
  \end{array}
\right))}{1+\frac12(\bm t, \bm0)\bm\Gamma\left(
  \begin{array}{c}
\bm t^\top\\
\bm0^\top\\
  \end{array}
\right)}=\frac{\exp(i\bm\mu\bm t^\top)}{1+\frac12\bm t\bm\Sigma\bm t^\top}.
\end{equation*}
Thus, ${\bm X}\sim\Laplace(\bm\mu,\bm\Sigma)$. The joint probability density function is (assuming $\det(\bm\Gamma)>0$)
\begin{equation*}
\begin{aligned}
p(\bm x,\bxk)&=\frac{2}{(2\pi)^p\sqrt{\det(\bm\Gamma)}}\left(\frac{(\bm x-\bm\mu, \bxk-\bm\mu)\bm\Gamma^{-1}\left(
  \begin{array}{c}
(\bm x-\bm\mu)^\top\\
(\bxk-\bm\mu)^\top\\
  \end{array}
\right)}{2}\right)^{\frac{1-p}{2}}\\
&\quad\times K_{1-p}(\sqrt{2(\bm x-\bm\mu, \bxk-\bm\mu)\bm\Gamma^{-1}\left(
  \begin{array}{c}
(\bm x-\bm\mu)^\top\\
(\bxk-\bm\mu)^\top\\
  \end{array}
\right)}),
\end{aligned}
\end{equation*}
where $K_{1-p}$ is the modified Bessel function of the second kind. Specifically, the conditional distribution $\bXk\mid  {\bm X}$ is a multivariate generalized hyperbolic distribution as in \citet{kotz2012laplace}.

If we use the representation in \citet{kotz2012laplace}, we can simplify things a lot. If ${\bm X}\sim\Laplace(\bm\mu,\bm\Sigma)$, it admits a representaton
\begin{equation*}
{\bm X}=\bm\mu+\sqrt{U}\bm Z, U\sim\Expo(1),\bm Z\sim\mathcal N(\bm0,\bm\Sigma)\text{ indenpendently}.
\end{equation*}
Similarly, we can first sample $U \mid  {\bm X}$, which has a density
\begin{equation*}
p(u \mid \bm x)=\frac{\exp(-u-\frac{({\bm x}-\bm\mu)\bm\Sigma^{-1}({\bm x}-\bm\mu)^\top}{2u})}{\sqrt{2({\bm x}-\bm\mu)\bm\Sigma^{-1}({\bm x}-\bm\mu)^\top}K_1(2({\bm x}-\bm\mu)\bm\Sigma^{-1}({\bm x}-\bm\mu)^\top)}, u>0.
\end{equation*}

It should be noted that this method easily generalizes to the asymmetric multivariate Laplace distribution, which, although not an elliptical distribution, admits similar representation
\begin{equation*}
{\bm X}=U\bm\mu+\sqrt{U}\bm Z, U\sim\Expo(1),\bm Z\sim\mathcal N(\bm0,\bm\Sigma)\text{ indenpendently}.
\end{equation*}

==> discussion/fixed-X.tex <==
\section{Fixed-X framework}
\subsection{Valid statistical testing}
Unlabeled data do not change the set of valid fixed-X tests.
\subsubsection{Necessity of conditioning on complete sufficient statistic}
Consider a valid level-$\alpha$ test conditional on $(X,Z)$. Let $R(X,Y,Z)$ be the rejection probability upon observing $(X,Y,Z)$, then
\begin{equation*}
\e_{H_0}[R(X,Y,Z)\mid \theta,X=x,Z=z]=\int R(x,y,z)f_{H_0}(y\mid \theta, z)\di y\le\alpha,\forall\theta,z,x.
\end{equation*}
Let $T(y,z)$ be a complete sufficient statistic for $\theta$, i.e., the conditional distribution $\mathcal L(Y\mid \theta,T(Y,Z),Z)$ is known and does not depend on $\theta$. Thus, $\e_{H_0}[R(X,Y,Z)\mid \theta,T(Y,Z),X,Z]$ is only a function of $T(X,Z)$, $X$ and $Z$. Denote it as $\alpha(T(Y,Z),X,Z)$.
\begin{enumerate}
\item If $R$ is based on an ancillary statistic, i.e., the distribution of $R$ does not depend on $\theta$, then by Basu's theorem, $R\ci T$, so $\alpha(T,X,Z)=\alpha(X,Z)$. It is then obvious that this term is smaller than $\alpha$.

\item If the test achieves level-$\alpha$ (almost) everywhere, then
\begin{equation*}
\begin{aligned}
\e_{H_0}[R(X,Y,Z)\mid \theta,X,Z]&=\e_{H_0}[\e_{H_0}[R(X,Y,Z)\mid \theta,T(Y,Z),X,Z]\mid \theta,X,Z]\\
&=\e_{H_0}[\alpha(T(Y,Z),X,Z)\mid \theta,X,Z]=\alpha,\forall\theta\Rightarrow\alpha(T,X,Z)\equiv\alpha.
\end{aligned}
\end{equation*}

\item In the Gaussian case with unknown variance and $n\le p$, suppose there is a set $S(x,z)$ such that when $t\in S(x,z)\subseteq\rr^p$, $\alpha(t,x,z)>\alpha+\varepsilon$, and there is positive mass in this set. That is, there exists $\theta$ and $\sigma$ such that if $Y\mid X,Z\sim\mathcal N(Z\theta,\sigma^2I_p)$ then $\p_\theta(T(Y,Z)\in S(X,Z)\mid X,Z)>0$. This would imply the set $S(x,z)$ has positive Lebesgue measure.

Without loss of generality, we assume every point $(t_1,t_2,\dots,t_p,t_\sigma)$ in $S(X,Z)$ is such that $Z^\top Y=t$ and $\|Y\|^2=t_\sigma^2$ has a solution $Y$. Since $Z$ is full rank, there exists $\theta\in\rr^p$ such that $Z\theta=Y$. Since $S$ has positive measure, almost every point inside has Lebesgue density $1$. For such a point, consider the nuisance parameters $(\theta,\sigma=\delta\to0)$. Most of the mass of $T$ under this set of parameters concentrate around $(t_1,t_2,\dots,t_p,t_\sigma)$, and eventually this would make $\e_{\theta,\delta}[\alpha(T,X,Z)\mid X,Z]>\alpha+\varepsilon/2$.
\end{enumerate}


If the type I error rate is not everywhere $\alpha$, consider the case with $Y\sim\mathcal N(\theta,1)$ with a single observation. Let $R(Y,X,Z)=\sqrt{3}\alpha\exp(-y^2)$. The complete sufficient statistic is $Y$ itself, and
\begin{equation*}
\int_\rr\sqrt{3}\alpha\exp(-y^2)\frac{1}{\sqrt{2\pi}}\exp(-(y-\theta)^2/2)\di y=\alpha\exp(-\theta^2/3)\le\alpha,\forall\theta.
\end{equation*}

If $n>p$, consider the test which rejects with probability $\alpha S\exp(1.1-S)$ (larger than $1$ when $S$ is around $1$), where $S$ is the sample variance (or residue) which follows a chi-squared distribution with degree of freedom $k=3$ and unknown positive scale $\sigma$. It can be shown that
\begin{equation*}
\e_{S\sim\sigma^2\chi_3^2}[\alpha S\exp(1.1-S)]=\frac{3e^{1.1}\alpha\sigma^2}{(1+2\sigma^2)^{\frac52}}\le\frac{9\sqrt{15}e^{1.1}\alpha }{125}<\alpha.
\end{equation*}

\subsubsection{Does unlabeled data help with choosing a test?}
We now study if unlabeled covariates can help in the fixed-X framework. % It is clear that if we know $F_X$, we do not need unlabeled samples, since we can generate them from $F_X$.
Clearly, even knowing exactly $F_X$ does not change the family of valid tests in the fixed-X framework (this is strictly stronger than having unlabeled samples from $F_X$).
\begin{thm}
Let
\begin{equation*}
R_\textnormal{fixed-X}=\{R(x,y):0\le R(x,y)\le1,\int R(x,y)p_\eta(y\mid x)\di y\le\alpha\text{ under }H_0,\forall\eta,x\}
\end{equation*}
be all valid fixed-X tests. Let $V_x:R_\textnormal{fixed-X}\to\rr[x]$ be a conditional rating function of tests, where $\rr[x]$ means all real functions of $x$. If $r_x\in R_\textnormal{fixed-X}$ maximizes $V_x(r)$ for every $x$, then $r(x,y)=r_x(x,y)$ maximizes $\e[V_X(r)]$, regardless of $X$'s distribution.
\end{thm}

\paragraph{Example.} Let $\pi$ be a prior distribution on the alternative space $H_1$ and let
\begin{equation*}
V_x(r)=\e_{\p\sim\pi}[\e_{(X,Y)\sim\p}[r(x,Y)\mid X=x]],
\end{equation*}
which is the expected power of the test $r(x,Y)$ given $X=x$. If $r_x$ maximizes this function, then $r(x,y)=r_x(x,y)$ maximizes the expected unconditional power of the test.

Minimaxity does not satisfy this. For example, consider the case where $X\sim\Bern(1/2)$. Let $Y\mid X\sim\Unif[0,1]$ under the null. Let $Y\mid X=0,\eta=\eta_1\sim Y\mid X=1,\eta=\eta_2\sim p_1$ and $Y\mid X=1,\eta=\eta_1\sim Y\mid X=0,\eta=\eta_2\sim p_2$, where
\begin{equation*}
p_1(y)=\left\{
\begin{aligned}
0.9,\quad &y\in[0,\frac12],\\
1.1,\quad &y\in[\frac12,1],
\end{aligned}
\right.
\end{equation*}
and
\begin{equation*}
p_2(y)=\left\{
\begin{aligned}
1.3,\quad &y\in[0,\frac12]\\
0.7,\quad &y\in[\frac12,1].
\end{aligned}
\right.
\end{equation*}
Now we show that a minimax test for $X=0$ which rejects with probability $r(y)$ when $Y=y$ must have power $\alpha$ under either alternative. Let $a=\int_0^{1/2}r(y)\di y\in[0,\alpha]$ and $b=\int_0^{1}r(y)\di y\in[a,\alpha]$. The power under $\eta=\eta_1$ is $\int_p^r(y)p_1(y)\di y=1.1b-0.2a$, while the power under $\eta=\eta_2$ is $\int_p^r(y)p_2(y)\di y=0.7b+0.6a$. Maximizing the minimum of these two gives $a=b/2$, and the power under each alternative is $b\le\alpha$. On the other hand, consider the test that rejects with probability $1$ if $Y\in[0,\alpha]$ and $0$ otherwise. If $\eta=\eta_1$, the marginal power of the test is
\begin{equation*}
\frac12\times\int_0^\alpha p_1(y)\di y+\frac12\times\int_0^\alpha p_2(y)\di y=1.1\alpha.
\end{equation*}
The same marginal power is obtained if $\eta=\eta_2$. This is strictly larger than $\alpha$.

For type I error, use fixed-X. For type II, use both.


\subsection{Optimal tests}
\subsubsection{Simple null versus simple alternative}
From the Neyman--Pearson lemma, unlabeled data clearly do not change the optimal test. Note that a model-X test might be optimal.

A simple example reveals that in finite samples, model-X test can be the optimal test. Let $X\sim f$. Let $Y\mid X\sim\Bern(g_\theta(X))$. Let $(X_i,Y_i)_{i=1}^n$ be i.i.d. copies of $(X,Y)$.
Assume
\begin{enumerate}
    \item there is a positive constant $M$ such that $X\mid|X|>M\eqd-X\mid|X|>M$ holds and $X\mid|X|\le M\eqd-X\mid|X|\le M$ doesn't hold.
    \item $g_0(x)\equiv1/2$;
    \item $g_\theta(x)+g_\theta(-x)\equiv1$;
    \item $g_\theta(x)$ is an increasing function of $x$ for $\theta>0$.
\end{enumerate}
Condition 1 ensures the marginal distribution of $Y$ depends on $\theta$, as opposed to the covariate $X$, whose marginal distribution does not depend on $\theta$. Consider testing $H_0:\theta=0$ versus $H_1:\theta=\theta_1>0$. Follow the Neyman--Pearson Lemma, the most powerful test is with rejection region of the form
\begin{equation*}
\prod_{i=1}^n(\ind_{Y_i=1}g_{\theta_1}(X_i)+\ind_{Y_i=0}g_{\theta_1}(-X_i))\ge c_\alpha.
\end{equation*}
For simplicity, let $Z_i=2Y_i-1$ be the symmetric version of $Y_i$, then the rejection region is
\begin{equation*}
\prod_{i=1}^ng_{\theta_1}(Z_iX_i)\ge c_\alpha.
\end{equation*}
Since $c_\alpha$ goes to $1$ as $\alpha\to0$, there is sufficiently small $\alpha$ such that $c_\alpha>g_{\theta_1}(M)$. For this $\alpha$, it's clear that
\begin{equation*}
\{x:\prod_{i=1}^ng_{\theta_1}(z_ix_i)\ge c_\alpha\}\subseteq\{x:|x_i|>M\},
\end{equation*}
for any fixed binary $\pm1$ sequence $z_1,z_2,\dots,z_n$. In this region $f$ is symmetric, so it's easy to see that the most powerful test has the correct size $\alpha$ conditional on $Z$. Put another way, the optimal test in this case is a model-X test.

\subsection*{General case with discrete $Y$}
Consider a simple null and a simple alternative. If $X$ is continuous and $Y$ is discrete with finite support, then for every $n$, for almost every $\alpha\in(0,1)$, we investigate the most powerful test conditional on $X$.

Let $\Lambda(\ndata{X},\ndata{Y})$ be the likelihood ratio statistic. Let $\mathcal Y$ be the support of $\ndata{Y}$, which is a finite set. Let $N=|\mathcal Y|$. Consider $\Pi$, all possible ranks of $\{\ndata{y}\in\mathcal Y:\Lambda(\ndata{X},\ndata{y})\}$, including ties. For each rank $\pi$, Let $A_\pi$ be the set of values of $\ndata{X}$ that give rise to this rank, e.g., $\ndata{X}\in A_\pi\Leftrightarrow \pi$. It's easy to see that $\{\pi\in\Pi:A_\pi\}$ is a partition of $\ndata{X}$'s support.

Consider a $\pi$ where $\p(\ndata{X}\in A_\pi)>0$. When $\pi$ is the rank, the rejection values of $\ndata{Y}$ is the top ones in this rank, followed by a possibly randomized rejection at the boundary to make size $\alpha$. Note that this rejection rule does not depend on the specific value of $\ndata{X}$, as $\ndata{X}$ and $\ndata{Y}$ are independent under the null. Obviously, for almost every $\alpha\in(0,1)$, a randomization is required. When a randomization is required, we can use the randomness in $\mathcal L(\ndata{X}\mid \ndata{X}\in A_\pi)$. Most of the time, we can expect an increased power.


\subsubsection{Testing scalar parameter under local alternatives}

==> discussion/model-X-knockoffs.tex <==
\section{Model-X knockoffs}


\subsection{}

Consider the case where the null feature statistics are i.i.d., then we can convert all feature importance statistics to a $p$-value $p_j=1-F(W_j)$, where $F$ is the distribution of a null feature statistic. And since $W_j$ is symmetric under the null, $F(x)+F(-x)=1$. The knockoff+ procedure from \citet{candes2018panning} becomes rejecting all $p$-values below $\tau_\text{KF}$, where
\begin{equation*}
\tau_\text{KF}=\max_{t\in[0,1]}\frac{1+\#\{j:p_j\ge 1-t\}}{\#\{j:p_j\le t\}}\le q.
\end{equation*}
On the other hand, the Benjamin--Hochberg procedure \citep{benjamini1995controlling} rejects all $p$-values below $\tau_\text{BH}$, where
\begin{equation*}
\tau_\text{BH}=\max_{t\in[0,1]}\frac{pt}{\#\{j:p_j\le t\}}\le q.
\end{equation*}

In \citet{storey2004strong}, a proposed correction of Benjamini-Hochberg is given below for a fixed parameter $\lambda\in[0,1)$. When $\lambda=0$, the standard BH procedure is recovered. The knockoffs procedure can be viewed as adaptively choosing $\lambda$.
\begin{equation*}
\tau_\text{Storey}^\lambda=\max_{t\in[0,1]}\frac{\frac{\#\{j:p_j>\lambda\}}{(1-\lambda)}t}{\#\{j:p_j\le t\}}\le q.
\end{equation*}

Clearly, one method does not dominate the other.

\subsection{Signal detection}
In this setting, we assume we have $p$ independent statistic $T_j\sim\mathcal N(\theta_j,1)$, with $\gamma$ fraction of $\theta_j$'s being $0$ and $(1-\gamma)$ being $h$.

Let $F_{\mu,\rho}$ be the distribution of $|X|-|Y|$, where
\begin{equation*}
\left(
  \begin{array}{c}
X\\
Y\\
  \end{array}
\right)\sim\mathcal N\left(\left(
  \begin{array}{c}
\mu\\
0\\
  \end{array}
\right),\left[
  \begin{array}{cc}
1 & \rho\\
\rho & 1\\
  \end{array}
\right]\right).
\end{equation*}
Suppose we have knockoff statistics $T_{j+p}$ from $\mathcal N(0,1)$, jointly normal with $T_j$ with correlation $\rho$ and independent of the other $T_j$'s.
Let the non-null $\beta_j$ be $\pm h$. It can be seen that the null $W_j=\sqrt n(\hat\beta_j-\hat\beta_{j+p})$ has distribution $(1-\rho^2)^{-1/2}F_{0,-\rho}$, and the non-null $W_j$ has distribution $(1-\rho^2)^{-1/2}F_{\pm h\sqrt{n(1-\rho^2)},-\rho}$. Equivalently, we can assume null $W_j\sim F_{0,\rho}$ and the non-null $W_j\sim F_{h\sqrt{n(1-\rho^2)},\rho}$. Clearly, we can expect high power occurs at a $\rho$ which makes $F_{h\sqrt{n(1-\rho^2)},\rho}$ different from $F_{0,\rho}$.
Note that
\begin{equation*}
\begin{aligned}
F_{\mu,\rho}(x)&=1-\p(\{X-Y\ge x,X+Y\ge x\}\cup\{X+Y\le-x,X-Y\le-x\})\\
&=1-\p(X-Y\ge x,X+Y\ge x)-\p(X+Y\le-x,X-Y\le-x)\\
&\quad+\p(X-Y\ge x,X+Y\ge x,X+Y\le-x,X-Y\le-x)\\
&=1-\Phi(\frac{\mu-x}{\sqrt{2(1+\rho)}})\Phi(\frac{\mu-x}{\sqrt{2(1-\rho)}})-\Phi(\frac{-\mu-x}{\sqrt{2(1+\rho)}})\Phi(\frac{-\mu-x}{\sqrt{2(1-\rho)}})\\
&\quad+\mathbb I(x<0)\left[\Phi(\frac{-x-\mu}{\sqrt{2(1+\rho)}})-\Phi(\frac{x-\mu}{\sqrt{2(1+\rho)}})\right]\left[\Phi(\frac{-x-\mu}{\sqrt{2(1-\rho)}})-\Phi(\frac{x-\mu}{\sqrt{2(1-\rho)}})\right]
\end{aligned}
\end{equation*}

Let
\begin{equation*}
\begin{aligned}
\tau_\text{KF}&=\min\{t>0:\frac{1+\#\{j:W_j\le-t\}}{\#\{j:W_j\ge t\}}\ge q\}\\
&\approx\min\{t>0:\frac{\gamma F_{0,\rho}(-t)+(1-\gamma)F_{h\sqrt{n(1-\rho^2)},\rho}(-t)}{\gamma F_{0,\rho}(-t)+(1-\gamma)(1-F_{h\sqrt{n(1-\rho^2)},\rho}(t))}\le q\},
\end{aligned}
\end{equation*}
and the power is $1-F_{h\sqrt{n(1-\rho^2)},\rho}(\tau_\text{KF})$.

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/rho0.pdf}
         \caption{$\rho=0$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.2}.pdf}
         \caption{$\rho=0.2$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.4}.pdf}
         \caption{$\rho=0.4$}
     \end{subfigure}
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.6}.pdf}
         \caption{$\rho=0.6$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.8}.pdf}
         \caption{$\rho=0.8$}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/rho/{rho0.99}.pdf}
         \caption{$\rho=0.99$}
     \end{subfigure}
        \caption{Comparison of $(1-\rho^2)^{-1/2}F_{h\sqrt{n(1-\rho^2)},\rho}$ (black) and $F_{0,\rho}$ (blue) with $h\sqrt{n}=3$.}
        \label{fig:compare-rhos}
\end{figure}
\begin{figure}[H]
    \centering
\includegraphics[width = 0.95\textwidth]{figures/p1000KFBH.pdf}
    \caption{Comparision of power at FDR level $0.1$; $p=1000$, $n=10p$.} 
    \label{figure:KF_power}
\end{figure}

\begin{lemma}
Let $\{G_n\}$ be a sequence of CDFs. If for every $t$, $G_n(t)\cip G(t)$, with $G$ being a (continuous) CDF, then the convergence in uniform in $t$, in the sense that
\begin{equation*}
\sup_{t}|G_n(t)-G(t)|\cip0.
\end{equation*}
\label{lemma:unif-conv-in-prob}
\end{lemma}
\begin{proof}
Take any $\varepsilon>0$. Find a finite number of points $x_1,x_2,\dots,x_N$ such that $G(x_1)\ge\varepsilon/2$, $G(x_{i})-G(x_{i-1})\le\varepsilon/2$ and $1-G(x_N)\le\varepsilon/2$. We have
\begin{equation*}
\p(\max_{1\le i\le N}|G_n(x_i)-G(x_i)|\le\varepsilon/2)\to1.
\end{equation*}
Now for any $x\in[x_{i-1},x_{i}]$ ($x_0=-\infty,x_{N+1}=\infty$), on the event $\max_{1\le i\le N}|G_n(x_i)-G(x_i)|\le\varepsilon/2$,
\begin{equation*}
G_n(x)\ge G_n(x_{i-1})\ge G(x_{i-1})-\varepsilon/2\ge G(x_i)-\varepsilon/2-\varepsilon/2\ge G(x)-\varepsilon,
\end{equation*}
\begin{equation*}
G_n(x)\le G_n(x_{i})\le G(x_{i})+\varepsilon/2\le G(x_{i-1})+\varepsilon/2+\varepsilon/2\le G(x)+\varepsilon.
\end{equation*}
Thus,
\begin{equation*}
\p(\sup_{t}|G_n(t)-G(t)|<\varepsilon)\ge\p(\max_{1\le i\le N}|G_n(x_i)-G(x_i)|\le\varepsilon/2)\to1.
\end{equation*}
\end{proof}

\begin{thm}
Assume $F_0$ and $F_1$ are two CDFs continuous on $\rr$ and
\begin{equation*}
\tau_\textnormal{KF}=\min\{t>0:g(t)\equiv\frac{\gamma F_0(-t)+(1-\gamma)(F_1(-t))}{\gamma (1-F_0(t))+(1-\gamma)(1-F_1(t))}\le q\}>0.
\end{equation*}
For almost every $q\in(0,1)$, the cutoff
\begin{equation*}
\tau_p=\min\{t>0:g_p(t)\equiv\frac{\#\{j:W_j<-t\}/p}{\#\{j:W_j>t\}/p}\le q\}
\end{equation*}
converges to $\tau_\textnormal{KF}$ in probability.
\label{theorem:cutoff-converge}
\end{thm}

\begin{proof}
First we observe that $g(\tau_\text{KF})=q$, or the maximum will be larger than $q$ because of $g$'s continuity. We further assume $g'(\tau_\text{KF})\ne0$, which is true for almost every $q$. It is easy to see that actually $g'(\tau_\text{KF})<0$. Take any $0<\varepsilon<\tau_\text{KF}$. There exists a point $\tau^*$ in $(\tau_\text{KF},\tau_\text{KF}+\varepsilon)$ such that $g(\tau^*)<q$. Then
\begin{equation*}
\begin{aligned}
\p(\tau_p<\tau_\text{KF}+\varepsilon)&\ge \p(\tau_p\le\tau^*)\\
&\ge\p(g_p(\tau^*)\le q)\\
&\ge\p(|g_p(\tau^*)-g(\tau^*)|<|g(\tau^*)-q|)\to1.
\end{aligned}
\end{equation*}
Pick $0<\delta_1<\min(1-F_0(\tau_\text{KF}-\varepsilon),1-F_1(\tau_\text{KF}-\varepsilon))$. Now observe that the function $\frac{\gamma x+(1-\gamma)y}{\gamma z+(1-\gamma)w}$ is continuous in $(x,y,z,w)$ on $\{(x,y,z,w):z,w\ge\min(1-F_0(\tau_\text{KF}-\varepsilon),1-F_1(\tau_\text{KF}-\varepsilon))-\delta_1\}$, and thus uniformly continuous. Pick $0<\delta_2<\delta_1$ such that whenever $(x,y,z,w)\in\{(x,y,z,w):z,w\ge\min(1-F_0(\tau_\text{KF}-\varepsilon),1-F_1(\tau_\text{KF}-\varepsilon))\}$ and $|x-x'|,|y-y'|,|z-z'|,|w-w'|<\delta_2$, $\frac{\gamma x+(1-\gamma)y}{\gamma z+(1-\gamma)w}-\frac{\gamma x'+(1-\gamma)y'}{\gamma z'+(1-\gamma)w'}|<\delta_3=\min\{g(t)-q:t\le\tau_\text{KF}-\varepsilon\}$. By Lemma~\ref{lemma:unif-conv-in-prob}, with probability converging to $1$, all the CDFs fall within a $\delta_2$-neighborhood around the limit CDFs, and by the previously mentioned uniform continuity, $|g_p(t)-g(t)|<\delta_3$ for $t\le\tau_\text{KF}-\varepsilon$. By the definition of $\delta_3$, this means with probability converging to $1$, $g_p(t)>q$ for all $t\le\tau_\text{KF}-\varepsilon$. Now we have
\begin{equation*}
\p(\tau_p>\tau_\text{KF}-\varepsilon)=\p(g_p(t)>q,\forall t\le\tau_\text{KF}-\varepsilon)\to1.
\end{equation*}
Combining the results, we have
\begin{equation*}
\lim_{p\to\infty}\p(|\tau_p-\tau_\text{KF}|<\varepsilon)=1.
\end{equation*}
\end{proof}

% \subsection{Best knockoff statistic?}
% Suppose $(X,\tilde X)\eqd(\tilde X,X)$ and $Y\ci \tilde X\mid X$. I conjecture that the best knockoff statistic is
% \begin{equation*}
% \ell(X=x,\tilde X=\tilde x,Y=y)-\ell(X=\tilde x,\tilde X=x,Y=y).
% \end{equation*}
% In multivariate testing, this is
% \begin{equation*}
% W_j=\ell(X_j=x_j,\tilde X_j=\tilde x_j,Y=y\mid \Xno{j},\tilde X_{\text{-}{j}})-\ell(X_j=\tilde x_j,\tilde X_j=x_j,Y=y\mid \Xno{j},\tilde X_{\text{-}{j}}).
% \end{equation*}
% The best means it gives the best $p$-value.

%\subsection{De-dependence for $W_j$ by removing conditional mean?}








\subsection{Low-dimensional case ($n\gg p$)}
% \subsubsection{Relationship of $n$ and $p$}
% We know that, with the non-null $\beta_j$'s being $h/\sqrt{n}$ and $\beta_0=\sqrt n\beta$,
% \begin{equation*}
% \sqrt n\hat\beta\sim\mathcal N\left(\beta_0,\sigma^2\left[
%   \frac1nX^\top X
% \right]^{-1}\right)\mid X.
% \end{equation*}
% Conditional on (an infinite sequence of) $X$, $W_p=\sqrt n\hat\beta$ follows a multivariate normal distribution $Q_p$. We want to establish that $Q_p$ is contiguous to $P_p=\mathcal N(\beta_0,\sigma^2I_p)$ almost surely under some conditions on the relationship between $n$ and $p$. The likelihood ratio is
% \begin{equation*}
% L_p=\sqrt{\det(X^\top X/n)}\exp\left(-\frac12w^\top(I_p-(X^\top X/n))w\right).
% \end{equation*}
% The log-likelihood is
% \begin{equation*}
% \ell_p=\frac12\log\det(X^\top X/n)-\frac12w^\top(I_p-(X^\top X/n))w.
% \end{equation*}
% By Theorem~12.3.1 in \citet{lehmann2006testing}, a sufficient condition is $L_p\cip 1$ under $P_p$. A sufficient condition is
% \begin{equation*}
% w^\top(I_p-(X^\top X/n))w\cip0\text{ and }\det(X^\top X/n)\to1.
% \end{equation*}
% For the former, since
% \begin{equation*}
% \begin{aligned}
% \p(|w^\top(I_p-(X^\top X/n))w|\ge\varepsilon)&\le\frac{\e[|w^\top(I_p-(X^\top X/n))w|^2]}{\varepsilon^2}\\
% &=\frac{\e[(\sum_{j=1}^p(\lambda_j-1)v_i^2)^2]}{\varepsilon^2}\\
% &=\frac{(\sum_{j=1}^p(\lambda_j-1))^2+2\sum_{j=1}^p(\lambda_j-1)^2}{\varepsilon^2}.
% \end{aligned}
% \end{equation*}
% % \begin{equation*}
% % \begin{aligned}
% % |w^\top(I_p-(X^\top X/n))w|\ge\varepsilon^2&\Rightarrow\|w\|^2\ge\frac{\varepsilon^2}{\max\{|\lambda_1|,|\lambda_2|,\dots,|\lambda_p|\}}\\
% % &\Rightarrow\frac{\|w\|^2}{p}\ge\frac{\varepsilon^2}{p\max\{|\lambda_1|,|\lambda_2|,\dots,|\lambda_p|\}},
% % \end{aligned}
% % \end{equation*}
% where $\lambda_{1:p}$ are eigenvalues of $X^\top X/n$ and $v_{1:p}\simiid\mathcal N(0,1)$.
% It converges to $0$ if $\sum_{j=1}^p(\lambda_j-1)^2$ and $\sum_{j=1}^p(\lambda_j-1)^2\to0$. To sum up, we have $Q_p$ is contiguous to $P_p$ if
% \begin{equation}
% \det(X^\top X/n)\to1,\sum_{j=1}^p(\lambda_j-1)\to0\text{ and }\sum_{j=1}^p(\lambda_j-1)^2\to0.
% \label{eq:knockoff-contiguity}
% \end{equation}
% Thus, we need $n$ to grow at such a rate that equation~\eqref{eq:knockoff-contiguity} holds. First we consider
% \begin{equation*}
% \sum_{j=1}^p(\lambda_j-1)=\trace(X^\top X)/n-p=\frac1n\sum_{i=1}^n\sum_{j=1}^p(X_{ij}^2-1).
% \end{equation*}
% Since $X_{ij}^2-1$ are i.i.d. with mean $0$ and variance $2$,
% \begin{equation*}
% \frac{|\sum_{i=1}^n\sum_{j=1}^p(X_{ij}^2-1)|}{\sqrt{np(\log(np))^\alpha}}\to0,a.s.,\forall\alpha>1.
% \end{equation*}
% If $n/p^{1+\delta}\to\infty$, $\delta>0$, $n/\sqrt{np(\log(np))^\alpha}\to\infty$ and thus $\sum_{j=1}^p(\lambda_j-1)\to0$ a.s.
% Second,
% \begin{equation*}
% \sum_{j=1}^p(\lambda_j-1)^2=\sum_{j=1}^p(\lambda_j^2-1)-2\sum_{j=1}^p(\lambda_j-1).
% \end{equation*}
% So we just need $\sum_{j=1}^p(\lambda_j^2-1)\to0$.
% \begin{equation*}
% \begin{aligned}
% \sum_{j=1}^p(\lambda_j^2-1)&=n^{-2}\trace((X^\top X)^2)-p\\
% &=n^{-2}\sum_{j=1}^p(\sum_{i=1}^nX_{ij}^2)^2-p+n^{-2}\sum_{j\ne k}(\sum_{i=1}^nX_{ij}X_{ik})^2.
% \end{aligned}
% \end{equation*}
% Let $n/p^{2+\delta}\to\infty$ for some $\delta>0$.
% \begin{equation*}
% \begin{aligned}
% \p(|n^{-2}\sum_{j=1}^p(\sum_{i=1}^nX_{ij}^2)^2-p|\ge p^{-\delta/4})&\le\frac{\e[|n^{-2}\sum_{j=1}^p(\sum_{i=1}^nX_{ij}^2)^2-p|^2]}{p^{-\delta/2}}\\
% &=\frac{\e[n^{-2}\sum_{j=1}^p(\sum_{i=1}^nX_{ij}^2)^2-p]^2+\Var(n^{-2}\sum_{j=1}^p(\sum_{i=1}^nX_{ij}^2)^2-p)}{p^{-\delta/2}}\\
% =&\frac{\frac{2p}n+\frac{8p(n+2) (n+3)}{n^3}}{p^{-\delta/2}}\sim p^{1+\delta/2}n^{-1}\ll p^{1+\delta/2}p^{-2-\delta}\sim p^{-1-\delta/2}.
% \end{aligned}
% \end{equation*}
% By Borel--Cantelli, this term converges to $0$ almost surely as $p\to\infty$.

% Let $n/p^{3+\delta}\to\infty$ for some $\delta>0$.
% \begin{equation*}
% \begin{aligned}
% \p(|n^{-2}\sum_{j\ne k}(\sum_{i=1}^nX_{ij}X_{ik})^2|\ge p^{-\delta/2})&\le\frac{\e[|n^{-2}\sum_{j\ne k}(\sum_{i=1}^nX_{ij}X_{ik})^2|]}{p^{-\delta/2}}\\
% &=\frac{\frac{p(p-1)}{n^2}\e[(\sum_{i=1}^nX_{i1}X_{i2})^2]}{p^{-\delta/2}}\\
% &=\frac{\frac{p(p-1)}{n^2}\e[\sum_{i=1}^nX_{i1}^2X_{i2}^2]}{p^{-\delta/2}}\text{ (cross terms have mean $0$)}\\
% =&\frac{\frac{p(p-1)}{n^2}n}{p^{-\delta/2}}\sim p^{2+\delta/2}n^{-1}\ll p^{2+\delta/2}p^{-3-\delta}\sim p^{-1-\delta/2}.
% \end{aligned}
% \end{equation*}
% By Borel--Cantelli, this term converges to $0$ almost surely as $p\to\infty$.

% Finally, by \citet{cai2015law},
% \begin{equation*}
% \begin{aligned}
% \p(|\det(X^\top X/n)|\ge p^{-\delta/4})&\le\frac{\e[|\det(X^\top X/n)|^2]}{p^{-\delta/2}}\\
% &\le2\frac{\e[(\det(X^\top X/n)-\tau_{n,p})^2]+\tau_{n,p}^2}{p^{-\delta/2}}\\
% &\le2\frac{-2\log(1-\frac pn)+\frac{10p}{3n(n-p)}+\tau_{n,p}^2}{p^{-\delta/2}},
% \end{aligned}
% \end{equation*}
% where
% \begin{equation*}
% \tau_{n,p}=\sum_{k=1}^p\log(1-\frac kn)+O(\frac1n).
% \end{equation*}
% Note that
% \begin{equation*}
% |\sum_{k=1}^p\log(1-\frac kn)|\le p\log(1-\frac pn)=\frac{p^2}{n}\frac{n}{p}\log(1-\frac pn)\sim \frac{p^2}n\cdot e\ll p^2p^{-3-\delta}\sim p^{-1-\delta},
% \end{equation*}
% so
% \begin{equation*}
% |\tau_{n,p}|=O(\max(p^{-1-\delta},n^{-1}))=O(\max(p^{-1-\delta},p^{-3-\delta}))=O(p^{-1-\delta}).
% \end{equation*}
% Thus,
% \begin{equation*}
% \frac{\tau_{n,p}^2}{p^{-\delta/2}}=O(p^{-2-2\delta})p^{\delta/2}=O(p^{-2-3\delta/2})
% \end{equation*}
% \begin{equation*}
% \frac{-\log(1-p/n)}{p^{-\delta/2}}\sim\frac{p^{1+\delta/2}}{n}\ll p^{1+\delta/2}p^{-3-\delta}\sim p^{-2-\delta/2}.
% \end{equation*}
% \begin{equation*}
% \frac{\frac{10p}{3n(n-p)}}{p^{-\delta/2}}\sim\frac{p^{1+\delta/2}}{n^{2}}\ll p^{1+\delta/2}p^{-6-2\delta}\sim p^{-5-3\delta/2},
% \end{equation*}

% % We have representation
% % \begin{equation*}
% % \log\det(X^\top X/n)\sim\sum_{k=1}^p\chi^2_{n-k+1}-p\log n.
% % \end{equation*}
% % We have tail bound \citep{laurent2000adaptive}
% % \begin{equation*}
% % \p(\chi_k^2\ge k+2\sqrt{kx}+2x)\le\exp(-x),x>0,
% % \end{equation*}
% % and
% % \begin{equation*}
% % \p(\chi_k^2\le k-2\sqrt{kx})\le\exp(-x),x>0,
% % \end{equation*}
% % Thus, for $t>0$,
% % \begin{equation*}
% % \begin{aligned}
% % \p(\log(\chi_k^2/k)\ge t)&=\p(\chi_k^2\ge ke^t)\\
% % &=\p(\chi_k^2\ge k+kt+kt^2/2+\dots)\\
% % &\le\p(\chi_k^2\ge k+kt+kt^2/2)\le\exp(-kt^2/4).
% % \end{aligned}
% % \end{equation*}
% % \begin{equation*}
% % \begin{aligned}
% % \p(\log(\chi_k^2/k)\le-t)&=\p(\chi_k^2\le ke^{-t})\\
% % &\le\exp(-k(1-e^{-t})^2/4).
% % \end{aligned}
% % \end{equation*}
% % I suspect that the second one also holds almost surely under $p=o(n^{1/3})$.\footnote{We know that if $p/n\to y>0$, $\max\{|\lambda_1|,|\lambda_2|,\dots,|\lambda_p|\}\to y+2\sqrt{y}$ a.s. \citep{bai1993limit}. Thus it seems to be true that $p\max\{|\lambda_1|,|\lambda_2|,\dots,|\lambda_p|\}\sim p^2/n+2\sqrt{p^3/n}$.}
% If $n/p^{3+\delta}\to\infty$ for some $\delta>0$, then equation~\eqref{eq:knockoff-contiguity} holds almost surely with respect to $X$, and for each $t$, $\frac{\#\{j:|w_j|-|w_{j+p}|\le t\}}{p}$ converges to the same limit under $P_p$ and the real distribution induced by OLS. The argument is if
% \begin{equation*}
% \lim_{p\to\infty}\p(f_p(Y,X)\ge\varepsilon\mid X)=0,\ a.s.\text{ (by contiguity)},
% \end{equation*}
% then
% \begin{equation*}
% \p(f_p(Y,X)\ge\varepsilon)=\e[\p(f_p(Y,X)\ge\varepsilon\mid X)]\to0
% \end{equation*}
% by the dominated convergence theorem.


% %Consider a linear model, and $(X_j,\tilde X_j)$ are i.i.d. normal with correlation $\rho_j$. Consider
% %\begin{equation*}
% %W_j=n^{-1/2}\sum_{i=1}^n[(X_{ij}-\tilde X_{ij})Y_i-\beta_j\sigma_j^2(1-\rho_j)]
% %\end{equation*}
% Let $\psi_j(X_j,\tilde X_j,Y)=(X_j-\tilde X_j)Y-\beta_j\sigma_j^2(1-\rho_j)$, and
% \begin{equation*}
% \begin{aligned}
% \e[\psi_j(X_j,\tilde X_j,Y)]&=\e[(X_{j}-\tilde X_{j})\sum_{\ell=1}^p\beta_\ell X_{\ell}-\beta_j\sigma_j^2(1-\rho_j)]\\
% &=\e[\beta_j(X_{j}-\tilde X_{j})X_{j}-\beta_j\sigma_j^2(1-\rho_j)]=0.
% \end{aligned}
% \end{equation*}

% For $j\ne k$,
% \begin{equation*}
% \begin{aligned}
% \Cov(\psi_j,\psi_k)&=\e[\Cov(\psi_j,\psi_k\mid X,\tilde X)]+\Cov(\e[\psi_j\mid X,\tilde X],\e[\psi_k\mid X,\tilde X])\\
% &=\e[(X_j-\tilde X_j)(X_k-\tilde X_k)\sigma^2]+\Cov((X_{j}-\tilde X_{j})\sum_{\ell=1}^p\beta_\ell X_{\ell},(X_{k}-\tilde X_{k})\sum_{\ell=1}^p\beta_\ell X_{\ell})\\
% &=0+\Cov((X_{j}-\tilde X_{j})(\beta_jX_j+\beta_kX_k),(X_{k}-\tilde X_{k})(\beta_jX_j+\beta_kX_k))\\
% &=\Cov((X_{j}-\tilde X_{j})\beta_jX_j,(X_{k}-\tilde X_{k})\beta_jX_j)+\Cov((X_{j}-\tilde X_{j})\beta_kX_k,(X_{k}-\tilde X_{k})\beta_kX_k)\\
% &=\e[\beta_j^2X_j^2(X_j-\tilde X_j)(X_k-\tilde X_k)]+\e[\beta_k^2X_k^2(X_j-\tilde X_j)(X_k-\tilde X_k)]\\
% &=\e[\beta_j^2X_j^2(X_j-\tilde X_j)]\e[X_k-\tilde X_k]+\e[\beta_k^2X_k^2(X_k-\tilde X_k)]\e[X_j-\tilde X_j]=0+0=0.
% \end{aligned}
% \end{equation*}

% \begin{equation*}
% \begin{aligned}
% \Var(\psi_j)&=\e[\Var(\psi_j\mid X,\tilde X)]+\Var(\e[\psi_j\mid X,\tilde X])\\
% &=\e[(X_j-\tilde X_j)^2\sigma^2]+\Var((X_{j}-\tilde X_{j})\sum_{\ell=1}^p\beta_\ell X_{\ell})\\
% &=2\sigma^2\sigma_j^2(1-\rho_j)+\e[(X_{j}-\tilde X_{j})^2(\sum_{\ell=1}^p\beta_\ell X_{\ell})^2]-\e[(X_{j}-\tilde X_{j})\sum_{\ell=1}^p\beta_\ell X_{\ell}]^2\\
% &=2\sigma^2\sigma_j^2(1-\rho_j)-\beta_j^2\sigma_j^4(1-\rho_j)^2+\e[\sum_{k,\ell}\beta_k\beta_\ell X_kX_\ell(X_{j}-\tilde X_{j})^2]\\
% &=2\sigma^2\sigma_j^2(1-\rho_j)-\beta_j^2\sigma_j^4(1-\rho_j)^2+\e[\sum_{k=1}^p\beta_k^2X_k^2(X_{j}-\tilde X_{j})^2]\\
% &=2\sigma^2\sigma_j^2(1-\rho_j)-\beta_j^2\sigma_j^4(1-\rho_j)^2+3\sigma_j^4(1-\rho_j)^2+\sigma_j^2(1-\rho_j)\sum_{k=1}^p\beta_k^2\sigma_k^2\\
% &=\sigma_j^2(1-\rho_j)[2\sigma^2+3\sigma_j^2(1-\rho_j)+\sum_{k\ne j}\beta_k^2\sigma_k^2]
% \end{aligned}
% \end{equation*}

% Consider the case where $(X,\tilde X)$ has mean zero and covariance $\left[
%   \begin{array}{cc}
% I & \rho I\\
% \rho I & I\\
%   \end{array}
% \right]$. Use the OLS estimates to get $W_j=\hat\beta_j-\hat\beta_{j+p}$ (use population precision matrix), we have
% \begin{equation*}
% W_j=\frac{n^{-1}}{1-\rho}\sum_{i=1}^n(X_{ij}-\tilde X_{ij})Y_i=\frac{n^{-1}}{1-\rho}\sum_{i=1}^n\psi_j(X_{ij},\tilde X_{ij},Y_i)+\beta_j.
% \end{equation*}
% Consider the case where the first $m_0=\gamma p$ covariates are null, and for the non-nulls $\beta_j=\frac h{\sqrt n}$. Then ,under some conditions (e.g., Theorem 11.1.6 in \citet{athreya2006measure}), we have
% \begin{equation*}
% \sqrt n\left(
%   \begin{array}{c}
% W_1\\
% W_2\\
% \vdots\\
% W_{m_0}\\
% W_{m_0+1}\\
% \vdots\\
% W_p\\
%   \end{array}
% \right)\cid\mathcal N\left(\left(
%   \begin{array}{c}
% 0\\
% 0\\
% \vdots\\
% 0\\
% h\\
% \vdots\\
% h\\
%   \end{array}
% \right),\frac{2\sigma^2+3(1-\rho)}{1-\rho}I_p\right).
% \end{equation*}

% Let $\varphi_j(X_j,Y)=X_jY$ and $\tilde\varphi_j(\tilde X_j,Y)=\tilde X_jY$.
% \begin{equation*}
% \e[\varphi_j]=\beta_j\sigma_j^2,\quad\e[\tilde\varphi_j]=\beta_j\sigma_j^2\rho_j.
% \end{equation*}

% If $j\ne k$,
% \begin{equation*}
% \begin{aligned}
% \Cov(\varphi_j,\varphi_k)&=\e[\Cov(\varphi_j,\varphi_k\mid X,\tilde X)]+\Cov(\e[\varphi_j\mid X,\tilde X],\e[\varphi_k\mid X,\tilde X])\\
% &=\e[X_jX_k\sigma^2]+\Cov(X_j\sum_{\ell=1}^p\beta_\ell X_{\ell},X_k\sum_{\ell=1}^p\beta_\ell X_{\ell})\\
% &=0+\sum_{\ell_1,\ell_2}\beta_{\ell_1}\beta_{\ell_2}\Cov(X_jX_{\ell_1},X_kX_{\ell_2})\\
% &=\beta_j\beta_k\Cov(X_j^2,X_k^2)+\beta_j\sum_{\ell_2\ne k}\beta_{\ell_2}\Cov(X_j^2,X_kX_{\ell_2})+\beta_k\sum_{\ell_1\ne j}\beta_{\ell_1}\Cov(X_jX_{\ell_1},X_k^2)\\
% &\quad+\sum_{\ell_1\ne j,\ell_2\ne k}\beta_{\ell_1}\beta_{\ell_2}\Cov(X_jX_{\ell_1},X_kX_{\ell_2})\\
% &=\beta_j\beta_k\Cov(X_jX_k,X_kX_j)=\beta_j\beta_k\sigma_j^2\sigma_k^2.
% \end{aligned}
% \end{equation*}

% \begin{equation*}
% \begin{aligned}
% \Cov(\varphi_j,\tilde\varphi_k)&=\e[\Cov(\varphi_j,\tilde\varphi_k\mid X,\tilde X)]+\Cov(\e[\varphi_j\mid X,\tilde X],\e[\tilde\varphi_k\mid X,\tilde X])\\
% &=\e[X_j\tilde X_k\sigma^2]+\Cov(X_j\sum_{\ell=1}^p\beta_\ell X_{\ell},\tilde X_k\sum_{\ell=1}^p\beta_\ell X_{\ell})\\
% &=0+\sum_{\ell_1,\ell_2}\beta_{\ell_1}\beta_{\ell_2}\Cov(X_jX_{\ell_1},\tilde X_kX_{\ell_2})=0.
% \end{aligned}
% \end{equation*}

% \begin{equation*}
% \begin{aligned}
% \Var(\varphi_j)&=\e[\Var(\varphi_j\mid X,\tilde X)]+\Var(\e[\varphi_j\mid X,\tilde X])\\
% &=\e[X_j^2\sigma^2]+\Var(X_j\sum_{\ell=1}^p\beta_\ell X_{\ell})\\
% &=\sigma_j^2\sigma^2+\sum_{\ell_1,\ell_2}\beta_{\ell_1}\beta_{\ell_2}\Cov(X_jX_{\ell_1},X_jX_{\ell_2})\\
% &=\sigma_j^2\sigma^2+\beta_j^2\sigma_j^4+\sum_{k=1}^p\beta_k^2\sigma_j^2\sigma_k^2.
% \end{aligned}
% \end{equation*}

% \begin{equation*}
% \begin{aligned}
% \Var(\tilde\varphi_j)&=\e[\Var(\tilde\varphi_j\mid X,\tilde X)]+\Var(\e[\tilde\varphi_j\mid X,\tilde X])\\
% &=\e[\tilde X_j^2\sigma^2]+\Var(\tilde X_j\sum_{\ell=1}^p\beta_\ell X_{\ell})\\
% &=\sigma_j^2\sigma^2+\sum_{\ell_1,\ell_2}\beta_{\ell_1}\beta_{\ell_2}\Cov(\tilde X_jX_{\ell_1},\tilde X_jX_{\ell_2})\\
% &=\sigma_j^2\sigma^2+\sum_{k=1}^p\beta_k^2\Cov(\tilde X_jX_k,\tilde X_jX_k)\\
% &=\sigma_j^2\sigma^2+\beta_j^2()\sum_{k=1}^p\beta_k^2\Cov(\tilde X_jX_k,\tilde X_jX_k)\\
% \end{aligned}
% \end{equation*}

% (TO BE CONTINUED)

Consider a model where the null $W_j$'s are i.i.d. with symmetric distribution, and the non-null $W_j$'s are i.i.d. with distribution $F_h$. Assume the number of nulls is $m_0$, and $\lim_{p\to\infty}m_0/p=\gamma\in(0,1)$.
\begin{equation*}
\begin{aligned}
\frac{1+\#\{j:p_j\ge 1-t\}}{\#\{j:p_j\le t\}}=&\frac{1+\#\{j\in\mathcal H_0:p_j\ge 1-t\}+\#\{j\notin\mathcal H_0:p_j\ge 1-t\}}{\#\{j\in\mathcal H_0:p_j\le t\}+\#\{j\notin\mathcal H_0:p_j\le t\}}\\
=&\frac{\frac1p+\frac{m_0}p\frac1{m_0}\sum_{j\in\mathcal H_0}\mathbb I(p_j\ge1-t)+\frac{p-m_0}p\frac1{p-m_0}\sum_{j\notin\mathcal H_0}\mathbb I(p_j\ge1-t)}{\frac{m_0}p\frac1{m_0}\sum_{j\in\mathcal H_0}\mathbb I(p_j\le t)+\frac{p-m_0}p\frac1{p-m_0}\sum_{j\notin\mathcal H_0}\mathbb I(p_j\le t)}\\
\to&\frac{\gamma t+(1-\gamma)(1-F_h(1-t))}{\gamma t+(1-\gamma)F_h(t)}, a.s.,
\end{aligned}
\end{equation*}
which is uniform over $t\in[0,1]$ as $p\to\infty$ by Glivenko--Cantelli theorem.
% Define the function in the last line as $g_\text{KF}(t)$.
% \begin{equation*}
% \begin{aligned}
% g'(t)=&\frac{\left[\gamma+(1-\gamma)F_h'(1-t)\right]\left[\gamma t+(1-\gamma)F_h(t)\right]-\left[\gamma+(1-\gamma)F_h'(t)\right]\left[\gamma t+(1-\gamma)(1-F_h(1-t))\right]}{\left[\gamma t+(1-\gamma)F_h(t)\right]^2}\\
% =&(1-\gamma)\frac{\gamma(F_h(t)+F_h(1-t)-1)+\gamma t(F_h'(1-t)-F_h'(t))+(1-\gamma)(F_h(t)F_h'(1-t)-F_h'(t)F_h(1-t))}{\left[\gamma t+(1-\gamma)F_h(t)\right]^2}.
% \end{aligned}
% \end{equation*}
% Assume the density of the alternative distribution $p_h(t)=F_h'(t)$ is decreasing in $t$. Then it follows that if 
Similarly,
\begin{equation*}
\frac{pt}{\#\{j:p_j\le t\}}\to\frac{t}{\gamma t+(1-\gamma)F_h(t)}, a.s.,
\end{equation*}
uniformly over $t\in[0,1]$ as $p\to\infty$. Assuming $F_h$ is concave, or $p_h(t)$ is decreasing, we have
\begin{equation*}
\frac{t}{\gamma t+(1-\gamma)F_h(t)}\ge\frac{\gamma t+(1-\gamma)(1-F_h(1-t))}{\gamma t+(1-\gamma)F_h(t)}.
\end{equation*}
Thus,
\begin{equation*}
\text{BH}_q=\{t\in[0,1]:\frac{t}{\gamma t+(1-\gamma)F_h(t)}\le q\}\subseteq\text{KF}_q=\{t\in[0,1]:\frac{\gamma t+(1-\gamma)(1-F_h(1-t))}{\gamma t+(1-\gamma)F_h(t)}\le q\}.
\end{equation*}
This implies
\begin{equation*}
\tau^\infty_\text{BH}=\max\text{BH}_q\le \tau^\infty_\text{KF}=\max\text{KF}_q.
\end{equation*}

In a simple model where the non-null $W_j$'s are i.i.d. $N(0,1)$ and the non-nulls are i.i.d. $N(\mu,1)$, we compare the power of the two procedure, both empirically and theoretically. This corresponds to the case of using OLS estimates as $W_j$ in low-dimensional settings ($n\gg p$).

% \begin{figure}[H]
%     \centering
% \includegraphics[width = 0.9\textwidth]{figures/BH.pdf}
%     \caption{Comparision of emprical and theoretical results of BH at FDR level $0.1$.} 
%     \label{figure:comp_BH}
% \end{figure}
% \begin{figure}[H]
%     \centering
% \includegraphics[width = 0.9\textwidth]{figures/KF.pdf}
%     \caption{Comparision of emprical and theoretical results of Knockoffs at FDR level $0.1$.} 
%     \label{figure:comp_KF}
% \end{figure}
% \begin{figure}[H]
%     \centering
% \includegraphics[width = 0.9\textwidth]{figures/theoretical.pdf}
%     \caption{Comparision of theoretical results of BH and Knockoffs at FDR level $0.1$.} 
%     \label{figure:comp_thoery}
% \end{figure}
\begin{figure}[H]
    \centering
\includegraphics[width = 0.5\textwidth]{figures/BHKF_power.pdf}
    \caption{Power comparision of BH and Knockoffs at FDR level $0.1$. The x-axis indicates the fraction of nulls ($\gamma$) and the darkness indicates the ratio of the Knockoffs power and the BH power where the effective signal strength ($h\sqrt{1-\kappa/2}$ for BH and $h\sqrt{1-\kappa}$ for Knockoffs) is such that the BH power is at the value indicated by the y-axis. Here, the BH procedure is given the advantage of knowing $\gamma$.}
    \label{figure:comp_BH_KF}
\end{figure}

\subsection{Moderate-dimensional case ($n\approx p$)}
% \citet{huang2008asymptotic} showed that under certain conditions, the bridge estimator in \eqref{eq:bridge} has the property of correctly selecting variables with probability converging to $1$, and the asymptotic distribution of the nonzero coefficients is the same as an oracle estimator which knows the true support.
% \begin{equation}
% \hat\beta=\text{argmin}_\beta\sum_{i=1}^n(Y_i-x_i^\top\beta)^2+\lambda_n\sum_{j=1}^{p_n}|\beta_j|^\gamma,\gamma\in(0,1).
% \label{eq:bridge}
% \end{equation}

% \subsection{Linear regression}
Let $2p/n\to\kappa\in(0,1)$. Let The OLS statistics with orthogonal Gaussian design ($\e[X^\top X/n]=I_p$) satisfy \citep{el2013robust,donoho2016high}
\begin{equation*}
\sqrt{\frac{1-\kappa}{\kappa}}(\hat\beta-\beta)=T_nU, T_n\ci U, U\sim\Unif(S^{2p-1}), T_n\cip1,
\end{equation*}
where $S^{2p-1}$ is the unit sphere in $\rr^{2p}$. Let $\beta_j\simiid(1-\gamma)\delta_{h/\sqrt n}+\gamma\delta_0$.
\begin{equation*}
W_j=|\hat\beta_j|-|\hat\beta_{j+p}|=|\beta_j+T_nU_j\sqrt{\frac{\kappa}{1-\kappa}}|-|T_nU_{j+p}\sqrt{\frac{\kappa}{1-\kappa}}|.
\end{equation*}
Consider
\begin{equation}
\begin{aligned}
\sqrt{\frac{2p(1-\kappa)}{\kappa}}W_j&=|\sqrt{n(1-\kappa)}\beta_j+T_n\sqrt{2p}U_j|-|T_n\sqrt{2p}U_{j+p}|\\
&=|\sqrt{n(1-\kappa)}\beta_j+\frac{T_n\sqrt{2p}}{V_{2p}}Z_j|-|\frac{T_n\sqrt{2p}}{V_{2p}}Z_{j+p}|\\
&\cid (1-\gamma) F_{h\sqrt{1-\kappa},0}+\gamma F_{0,0}\text{ (Slutsky's theorem)},
\end{aligned}
\label{eq:conv-in-dist-W}
\end{equation}
and
\begin{equation}
\sqrt{\frac{2p(1-\kappa)}{\kappa}}(W_j,W_k)\cid \text{two i.i.d. }[(1-\gamma) F_{h\sqrt{1-\kappa},0}+\gamma F_{0,0}]\text{'s ($j\ne k$, Slutsky's theorem)}
\label{eq:conv-in-dist-W2}
\end{equation}
similarly.
% The inference via knockoffs with $W_j$ does not change if we multiply all $W_j$'s with an independent $\chi_{2p}$ random variable $V_{2p}$ and $\sqrt{\frac{1-\kappa}\kappa}T_n$. Thus, it is equivalent to consider
% \begin{equation*}
% W_j=|\frac{V_{2p}}{T_n}\sqrt{\frac{1-\kappa}\kappa}\beta_j+Z_j|-|Z_{j+p}|,
% \end{equation*}
% where $Z\sim\mathcal N(0,I_{2p})$, and $V_{2p},T_n,Z$ are mutually independent.
Now we rescale $W_j$ in the above way and consider $\#\{j:W_j\le t\}/p$ for a $t\in\rr$.
\begin{equation*}
\begin{aligned}
&\p(|\#\{j:W_j\le t\}/p-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t))|>\varepsilon)\\
&\le\frac{\e[(\#\{j:W_j\le t\}-p((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))^2]}{p^2\varepsilon^2}\\
&=\frac{\e[(\sum_{j=1}^p\mathbb I(W_j\le t)-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t))))^2]}{p^2\varepsilon^2}\\
&=\frac{1}{p^2\varepsilon^2}\big(p\e[(\mathbb I(W_1\le t)-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))^2]+p(p-1)\times\\
&\quad\quad\e[(\mathbb I(W_1\le t)-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))(\mathbb I(W_2\le t)-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))]\big)\\
&=\frac{1}{p^2\varepsilon^2}\big(p\left(\p(W_1\le t)\p(W_1>t)+(\p(W_1\le t)-(1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))^2\right)+p(p-1)\times\\
&\quad\quad\e[(\mathbb I(W_1\le t)-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))(\mathbb I(W_2\le t)-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))]\big)\\
&\le\frac{1}{p\varepsilon^2}+\frac{\e[(\mathbb I(W_1\le t)-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))(\mathbb I(W_2\le t)-((1-\gamma) F_{h\sqrt{1-\kappa},0}(t)+\gamma F_{0,0}(t)))]\big)}{\varepsilon^2}.
\end{aligned}
\end{equation*}
The first term goes to $0$ as $p\to\infty$, and the second term goes to zero due to the convergence in distribution \eqref{eq:conv-in-dist-W2}.

\begin{thm}
In a linear regression with design matrix having $i.i.d.$ $\mathcal N(0,1)$ entries, and $\beta_j\simiid(1-\gamma)\delta_{h/\sqrt n}+\gamma\delta_0$, $\gamma\in(0,1)$, $2p/n\to\kappa\in(0,1)$, then for almost every FDR level $q\in(0,1)$, the model-X knockoff procedure that uses absolute OLS difference statistic and independent knockoff variables has power converging in probability to
\begin{equation*}
1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)}),
\end{equation*}
where
\begin{equation*}
\tau^{(q)}=\min\{t>0:g(t)\equiv\frac{\gamma F_{0,0}(-t)+(1-\gamma)(F_{h\sqrt{1-\kappa},0}(-t))}{\gamma (1-F_{0,0}(t))+(1-\gamma)(1-F_{h\sqrt{1-\kappa},0}(t))}\le q\}.
\end{equation*}
\label{theorem:KF-ols}
\end{thm}

\begin{proof}
We need to prove that
\begin{equation*}
\frac{\#\{j:\beta_j\ne0,W_j\le\tau_p\}/p}{\#\{j:\beta_j\ne0\}/p}\cip1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)}).
\end{equation*}
The denominator converges in probability to $1-\gamma$ by the weak law of large numbers. Now we need to prove the numerator converges to $(1-\gamma)(1-F_{h\sqrt{1-\kappa},0}(\tau_q))$ in probability. By Markov inequality,
\begin{equation*}
\begin{aligned}
&\p(|\#\{j:\beta_j\ne0,W_j\ge \tau_p\}/p-(1-\gamma)(1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)}))|>\varepsilon)\\
&\le\frac{\e[(\#\{j:\beta_j\ne0,W_j\ge \tau_p\}-p(1-\gamma)(1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)})))^2]}{p^2\varepsilon^2}\\
&=\frac{\e[(\mathbb I(\beta_1\ne0,W_1\ge \tau_p)-(1-\gamma)(1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)})))^2]}{p\varepsilon^2}+\frac{p-1}{p\varepsilon^2}\times\\
&\e[(\mathbb I(\beta_1\ne0,W_1\ge \tau_p)-(1-\gamma)(1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)})))(\mathbb I(\beta_2\ne0,W_2\ge \tau_p)-(1-\gamma)(1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)})))].
\end{aligned}
\end{equation*}
We just need to show the second term goes to $0$, which would follow from
\begin{equation*}
\p(\beta_1\ne0,W_1\ge \tau_p)\to(1-\gamma)(1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)}))
\end{equation*}
and
\begin{equation*}
\p(\beta_1\ne0,W_1\ge \tau_p,\beta_2\ne0,W_2\ge \tau_p)\to(1-\gamma)^2(1-F_{h\sqrt{1-\kappa},0}(\tau^{(q)}))^2.
\end{equation*}
By writing $W_1\ge\tau_p$ as $W_1-\tau_p\ge0$ and noticing that $\tau_p\cip\tau^{(q)}\mid\beta_1,\beta_2$, the results follow from Slutsky's theorem.
\end{proof}

\begin{thm}
Assume the conditions of Theorem~\ref{theorem:KF-ols}. For almost every FDR level $q\in(0,1)$, the Benjamini-Hochberg procedure using absolute OLS statistic has power converging in probability to
\begin{equation*}
\Phi(h\sqrt{1-\kappa/2}-\tau^{(q)})+\Phi(-\tau^{(q)}-h\sqrt{1-\kappa/2}),
\end{equation*}
where
\begin{equation*}
\tau^{(q)}=\min\{t>0:\frac{2\Phi(-t)}{\gamma 2\Phi(-t)+(1-\gamma)(\Phi(h\sqrt{1-\kappa/2}-\tau^{(q)})+\Phi(-\tau^{(q)}-h\sqrt{1-\kappa/2}))}\le q\}.
\end{equation*}
\end{thm}

\subsection{High-dimensional case ($n<p$)}

In \citet{bayati2011lasso}, we have almost surely,
\begin{equation}
\lim_{p\to\infty}\frac1p\sum_{j=1}^p\psi(\hat\beta_j,\beta_{0,j})
=\e[\psi(\eta(B_0+\tau_*Z;\theta_*),B_0)],
\label{eq:lasso-amp-dist}
\end{equation}
where $Z\sim N(0,1)$ independent of $B_0\sim p_{B_0}$, $\tau_*=\tau_*(\alpha(\lambda))$, $\theta_*=\alpha(\lambda)\tau_*$.
Let $\{\beta_{2j-1}\}_{j=1}^\infty$ converges in distribution to $\gamma\delta_0+(1-\gamma)\delta_{h}$. and $\beta_{2j}=0$. Let $F_0$ and $F_1$ be the CDFs of $|\eta(\tau_*Z;\theta_*)|$ and $|\eta(h+\tau_*Z;\theta_*)|$.
\begin{equation*}
\begin{aligned}
&\e[\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_{2j-1}|-|\hat\beta_{2j}|>t)]\\
&=\p(|\hat\beta_{2J-1}|-|\hat\beta_{2J}|>t)\text{ ($J\sim\Unif(\{1,2,\dots,p\})$)}\\
&=\p(|\hat\beta_{2J-1}|-|\hat\beta_{2J'}|>t)\text{ ($J,J'\simiid\Unif(\{1,2,\dots,p\})$, exchangeability)}.
\end{aligned}
\end{equation*}
We know the limit of this probability if we can show that
\begin{equation*}
(|\hat\beta_{2J-1}|,|\hat\beta_{2J'}|)\cid(\gamma F_0+(1-\gamma)F_1,F_0)\text{ with independent coordinates}.
\end{equation*}

\begin{equation*}
\p(|\hat\beta_{2J-1}|\le s,|\hat\beta_{2J'}|\le t)=\e[\hat F^\text{odd}_p(s)\hat F^\text{even}_p(t)],
\end{equation*}
where
\begin{equation*}
\hat F^\text{odd}_p(s)=\frac1p\sum_{j=1}^p\mathbb I(|\hat\beta_{2j-1}|\le s),\hat F^\text{even}_p(t)=\frac1p\sum_{j=1}^p\mathbb I(|\hat\beta_{2j}|\le t).
\end{equation*}
We need these two terms to converge in probability, which would give us asymptotic independence of $|\hat\beta_{2J-1}|$ and $|\hat\beta_{2J'}|$ by convergence of CDF via bounded convergence theorem. By exchangeability,
\begin{equation*}
\sum_{j=1}^p\mathbb I(|\hat\beta_{2j}|\le t)\mid\hat\beta\sim\text{Hypergeometric}(p+p\gamma_p,{\sum_{j=1}^{2p}\mathbb I(|\hat\beta_{j}|\le t,\beta_j=0)},p).
\end{equation*}
Here,
\begin{equation*}
\gamma_p=\frac{\#\{j\in[p]:\beta_{2j-1}=0\}}{p}\to\gamma.
\end{equation*}
The hypergeometric distribution diviede by $p$ has mean
\begin{equation*}
\frac{\sum_{j=1}^{2p}\mathbb I(|\hat\beta_{j}|\le t,\beta_j=0)}{p+p\gamma_p}
\end{equation*}
and variance
\begin{equation*}
\frac{\sum_{j=1}^{2p}\mathbb I(|\hat\beta_{j}|\le t,\beta_j=0)}{p+p\gamma_p}\left(1-\frac{\sum_{j=1}^{2p}\mathbb I(|\hat\beta_{j}|\le t,\beta_j=0)}{p+p\gamma_p}\right)\frac{\gamma_p}{p-1}.
\end{equation*}

% \begin{lemma}
% \begin{equation*}
% \frac{1}{2p}\sum_{j=1}^{2p}\mathbb I(|\hat\beta_{j}|\le t,\beta_j=0)\to\frac{\gamma+1}{2}\p(|\eta(\tau_*Z;\theta_*)|\le t), a.s.
% \end{equation*}
% \label{lemma:lasso-amp-even}
% \end{lemma}

% \begin{proof}
% Let $\phi(x,y)=\mathbb I(|x|\le t,|y|\le\frac h2)$, and the left hand side is then
% \begin{equation*}
% \frac{1}{2p}\sum_{j=1}^{2p}\phi(\hat\beta_j,\beta_j).
% \end{equation*}
% Take
% \begin{equation*}
% \phi_{1,n}(x,y)=1-\max(1,n\times\inf_{|z|\le t,|w|\le h/2}\|(z,w)-(x,y)\|),
% \end{equation*}
% and
% \begin{equation*}
% \phi_{2,n}(x,y)=\min(1,n\times\inf_{|z|\ge t,|w|\ge h/2}\|(z,w)-(x,y)\|).
% \end{equation*}
% It is clear that
% \begin{equation*}
% \phi_{2,n}(x,y)\le\phi(x,y)\le\phi_{1,n}(x,y),
% \end{equation*}
% \begin{equation*}
% \phi_{1,n}(x,y),\phi_{2,n}(x,y)\to\phi(x,y),
% \end{equation*}
% and for each $n>0$, $\phi_{1,n}$ and $\phi_{2,n}$ are uniformly continuous and equation~\eqref{eq:lasso-amp-dist} holds. Since in our case, $B_0\sim\frac{\gamma+1}2\delta_0+\frac{1-\gamma}2\delta_h$ can only take value $0$ or $h$, when $n$ is sufficiently large,
% \begin{equation}
% \begin{aligned}
% \e[\phi_{1,n}(\eta(B_0+\tau_*Z;\theta_*),B_0)]&=\p(B_0=0)\e[\phi_{1,n}(\eta(\tau_*Z;\theta_*),0)]\to\frac{\gamma+1}2\e[\phi(\eta(\tau_*Z;\theta_*),0)]\\
% \e[\phi_{2,n}(\eta(B_0+\tau_*Z;\theta_*),B_0)]&=\p(B_0=0)\e[\phi_{2,n}(\eta(\tau_*Z;\theta_*),0)]\to\frac{\gamma+1}2\e[\phi(\eta(\tau_*Z;\theta_*),0)]
% \end{aligned}
% \label{eq:sup-inf}
% \end{equation}
% by the bounded convergence theorem. Since
% \begin{equation*}
% \frac{1}{2p}\sum_{j=1}^{2p}\phi_{2,n}(\hat\beta_j,\hat\beta)\le\frac{1}{2p}\sum_{j=1}^{2p}\phi(\hat\beta_j,\hat\beta)\le\frac{1}{2p}\sum_{j=1}^{2p}\phi_{1,n}(\hat\beta_j,\hat\beta),
% \end{equation*}
% we have, for each $n$ large enough,
% \begin{equation*}
% \limsup_{p\to\infty}\frac{1}{2p}\sum_{j=1}^{2p}\phi(\hat\beta_j,\hat\beta)\le\lim_{p\to\infty}\frac{1}{2p}\sum_{j=1}^{2p}\phi_{1,n}(\hat\beta_j,\hat\beta)=\e[\phi_{1,n}(\eta(\tau_*Z;\theta_*),0)]
% \end{equation*}
% and
% \begin{equation*}
% \liminf_{p\to\infty}\frac{1}{2p}\sum_{j=1}^{2p}\phi(\hat\beta_j,\hat\beta)\ge\lim_{p\to\infty}\frac{1}{2p}\sum_{j=1}^{2p}\phi_{2,n}(\hat\beta_j,\hat\beta)=\e[\phi_{2,n}(\eta(\tau_*Z;\theta_*),0)].
% \end{equation*}
% The result then follows from equations~\eqref{eq:sup-inf}.

% {\color{red} We can generalize this to $\beta_j\simiid\gamma\delta_0+(1-\gamma)f$ with $f$ having no mass at $0$. Just need to show that
% \begin{equation*}
% \lim_{\varepsilon\to0}\lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,|\beta_j|\le\varepsilon)=\lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,|\beta_j|=0),
% \end{equation*}
% while the difference is
% \begin{equation*}
% \lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,0<|\beta_j|\le\varepsilon)\le\lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(0<|\beta_j|\le\varepsilon)\to0\text{ as }\varepsilon\to0.
% \end{equation*}
% }
% \end{proof}

\begin{lemma}
Let the empirical distribution of $\beta_j$ converge to $\gamma\delta_0+(1-\gamma)f$, where $f$ is a distribution with no point mass at $0$. Then
\begin{equation*}
\frac{1}{p}\sum_{j=1}^{p}\mathbb I(|\hat\beta_{j}|\le t,\beta_j=0)\to\gamma\p(|\eta(\tau_*Z;\theta_*)|\le t), a.s.,
\end{equation*}
for any $t\ge0$.
\label{lemma:lasso-amp-even}
\end{lemma}

\begin{proof}
For $t,\varepsilon>0$, let $\phi(x,y)=\mathbb I(|x|\le t,|y|\le\varepsilon)$. Take
\begin{equation*}
\phi_{1,n}(x,y)=1-\max(1,n\times\inf_{|z|\le t,|w|\le\varepsilon}\|(z,w)-(x,y)\|),
\end{equation*}
and
\begin{equation*}
\phi_{2,n}(x,y)=\min(1,n\times\inf_{|z|\ge t,|w|\ge\varepsilon}\|(z,w)-(x,y)\|).
\end{equation*}
It is clear that
\begin{equation*}
\phi_{2,n}(x,y)\le\phi(x,y)\le\phi_{1,n}(x,y),
\end{equation*}
\begin{equation*}
\phi_{1,n}(x,y),\phi_{2,n}(x,y)\to\phi(x,y),
\end{equation*}
and for each $n>0$, $\phi_{1,n}$ and $\phi_{2,n}$ are uniformly continuous and equation~\eqref{eq:lasso-amp-dist} holds.
\begin{equation}
\begin{aligned}
&\e[\phi_{1,n}(\eta(B_0+\tau_*Z;\theta_*),B_0)]\\
&=\p(B_0=0)\e[\phi_{1,n}(\eta(\tau_*Z;\theta_*),0)]+\p(0<|B_0|\le\varepsilon)\e[\phi_{1,n}(\eta(B_0+\tau_*Z;\theta_*),B_0)\mid0<|B_0|\le\varepsilon]\\
&\to\gamma\e[\phi(\eta(\tau_*Z;\theta_*),0)]+\p(0<|B_0|\le\varepsilon)\e[\phi(\eta(B_0+\tau_*Z;\theta_*),B_0)\mid0<|B_0|\le\varepsilon]\\
&\e[\phi_{2,n}(\eta(B_0+\tau_*Z;\theta_*),B_0)]\\
&=\p(B_0=0)\e[\phi_{2,n}(\eta(\tau_*Z;\theta_*),0)]+\p(0<|B_0|\le\varepsilon)\e[\phi_{2,n}(\eta(B_0+\tau_*Z;\theta_*),B_0)\mid0<|B_0|\le\varepsilon]\\
&\to\gamma\e[\phi(\eta(\tau_*Z;\theta_*),0)]+\p(0<|B_0|\le\varepsilon)\e[\phi(\eta(B_0+\tau_*Z;\theta_*),B_0)\mid0<|B_0|\le\varepsilon]
\end{aligned}
\label{eq:sup-inf}
\end{equation}
by the bounded convergence theorem. Since
\begin{equation*}
\frac{1}{2p}\sum_{j=1}^{2p}\phi_{2,n}(\hat\beta_j,\beta_j)\le\frac{1}{2p}\sum_{j=1}^{2p}\phi(\hat\beta_j,\beta_j)\le\frac{1}{2p}\sum_{j=1}^{2p}\phi_{1,n}(\hat\beta_j,\beta_j),
\end{equation*}
we have, for each $n$ large enough,
\begin{equation*}
\limsup_{p\to\infty}\frac{1}{2p}\sum_{j=1}^{2p}\phi(\hat\beta_j,\beta_j)\le\lim_{p\to\infty}\frac{1}{2p}\sum_{j=1}^{2p}\phi_{1,n}(\hat\beta_j,\beta_j)=\e[\phi_{1,n}(\eta(\tau_*Z;\theta_*),0)]
\end{equation*}
and
\begin{equation*}
\liminf_{p\to\infty}\frac{1}{2p}\sum_{j=1}^{2p}\phi(\hat\beta_j,\beta_j)\ge\lim_{p\to\infty}\frac{1}{2p}\sum_{j=1}^{2p}\phi_{2,n}(\hat\beta_j,\beta_j)=\e[\phi_{2,n}(\eta(\tau_*Z;\theta_*),0)].
\end{equation*}
Then it follows from equations~\eqref{eq:sup-inf} that
\begin{equation*}
\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,|\beta_j|\le\varepsilon)\to\gamma\e[\phi(\eta(\tau_*Z;\theta_*),0)]+\p(0<|B_0|\le\varepsilon)\e[\phi(\eta(B_0+\tau_*Z;\theta_*),B_0)\mid0<|B_0|\le\varepsilon].
\end{equation*}
Now we want to show
\begin{equation*}
\lim_{\varepsilon\to0}\lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,|\beta_j|\le\varepsilon)=\lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,|\beta_j|=0),
\end{equation*}
while the difference is
\begin{equation*}
\lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,0<|\beta_j|\le\varepsilon)\le\lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(0<|\beta_j|\le\varepsilon),
\end{equation*}
which converges to $0$ as $\varepsilon\to0$.

Now we have shown for any $t>0$,
\begin{equation*}
\lim_{p\to\infty}\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,|\beta_j|=0)=\gamma\p(|\eta(\tau_*Z;\theta_*)|\le t).
\end{equation*}
\begin{equation*}
\begin{aligned}
\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le t,|\beta_j|=0)-\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|\le 0,|\beta_j|=0)&=\frac1p\sum_{j=1}^p\mathbb I(0<|\hat\beta_j|\le t,|\beta_j|=0)\\
&\le\frac1p\sum_{j=1}^p\mathbb I(0<|\hat\beta_j|\le t).
\end{aligned}
\end{equation*}
Using equation~(4) in \citet{bogdan2013supplementary}, we can show
\begin{equation*}
\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_j|= 0,|\beta_j|=0)\cip\gamma\p(|\eta(\tau_*Z;\theta_*)|=0).
\end{equation*}
\end{proof}

By Lemma~\ref{lemma:lasso-amp-even}, letting $B_p$ denote $\frac{1}{2p}\sum_{j=1}^{2p}\mathbb I(|\hat\beta_{j}|\le t,\beta_j=0)$,
\begin{equation*}
\e[\frac{1}{2p}\sum_{j=1}^{2p}\mathbb I(|\hat\beta_{2j}|\le t)]=\frac{2}{1+\gamma_p}\e[B_p]\to\p(|\eta(\tau_*Z;\theta_*)|\le t)
\end{equation*}
by the bounded convergence theorem.
\begin{equation*}
\begin{aligned}
\Var[\frac{1}{p}\sum_{j=1}^{p}\mathbb I(|\hat\beta_{2j}|\le t)]&=\e[\frac{2B_p}{1+\gamma_p}(1-\frac{2B_p}{1+\gamma_p})\frac{\gamma_p}{p-1}]+\Var[\frac{2B_p}{1+\gamma_p}]\\
&\le\frac{\gamma_p}{p-1}+\frac{4}{(1+\gamma_p)^2}\Var[B_p]\to0,
\end{aligned}
\end{equation*}
where $\Var[B_p]\to0$ by the bounded convergence theorem. Now we have shown
\begin{equation*}
\hat F^\text{even}_p(t)\cip\p(|\eta(\tau_*Z;\theta_*)|\le t),
\end{equation*}
%which is uniform for all $t\ge0$ by an argument similar to Lemma~\ref{lemma:unif-conv-in-prob};
convergence of $\hat F^\text{odd}_p(s)$ follows from
\begin{equation*}
\hat F^\text{odd}_p(s)=2\times\frac{1}{2p}\sum_{j=1}^{2p}\mathbb I(|\hat\beta_j|\le s)-\hat F^\text{even}_p(s).
\end{equation*}
Now we just need to analyze the following for Markov inequality.
\begin{equation*}
\begin{aligned}
\e[(\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_{2j-1}|-|\hat\beta_{2j}|>t))^2]&=\frac1p\p(|\hat\beta_{2J_1-1}|-|\hat\beta_{2J_1'}|>t)\\
&\quad+\frac{p-1}p\p(|\hat\beta_{2J_1-1}|-|\hat\beta_{2J_1'}|>t,|\hat\beta_{2J_2-1}|-|\hat\beta_{2J_2'}|>t),
\end{aligned}
\end{equation*}
where
\begin{equation*}
(J_1,J_1',J_2,J_2')\simiid\Unif(\{(i,j,k,\ell)\in[p]^4:i\ne k,j\ne \ell\}).
\end{equation*}
We can evaluate this by showing that asymptotically $(|\hat\beta_{2J_1-1}|,|\hat\beta_{2J_1'}|,|\hat\beta_{2J_2-1}|,|\hat\beta_{2J_2'}|)$ converges in distribution to four independent random variables.
\begin{equation*}
\p(|\hat\beta_{2J_1-1}|\le s,|\hat\beta_{2J_1'}|\le s',|\hat\beta_{2J_2-1}|\le t,|\hat\beta_{2J_2'}|\le t')=\e[\hat F_\text{odd}(s)\hat F_\text{even}(t)(\hat F_\text{odd}(s')-\frac1p)(\hat F_\text{even}(t')-\frac1p)],
\end{equation*}
assuming $s\le s'$ and $t\le t'$ without loss of generality. The desired result follows immediately. We would now be able to claim convergence in probability for
\begin{equation*}
\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_{2j-1}|-|\hat\beta_{2j}|>t).
\end{equation*}
For
\begin{equation*}
\frac{1}{p}\sum_{j=1}^p\mathbb I(|\hat\beta_{2j-1}|-|\hat\beta_{2j}|>t,\beta_{2j-1}=0),
\end{equation*}
let $N_p=\{j\in[p]:\beta_{2j-1}=0\}$. We just need to show that
\begin{equation*}
(|\hat\beta_{2J_1-1}|,|\hat\beta_{2J_1'}|,|\hat\beta_{2J_2-1}|,|\hat\beta_{2J_2'}|)\cid(F_0,F_0,F_0,F_0)\text{ with independent coordinates},
\end{equation*}
where
\begin{equation*}
(J_1,J_1',J_2,J_2')\sim\Unif(\{(i,j,k,\ell)\in N_p^4: i\ne k,j\ne \ell\}).
\end{equation*}
Note that
\begin{equation*}
\begin{aligned}
\p(|\hat\beta_{2J_1-1}|\le s,|\hat\beta_{2J_1'}|\le s',|\hat\beta_{2J_2-1}|\le t,|\hat\beta_{2J_2'}|\le t')\\
=\e[\hat F_\text{odd null}(s)\hat F_\text{even null}(t)(\hat F_\text{odd null}(s')-\frac1{p\gamma_p})(\hat F_\text{even null}(t')-\frac1{p\gamma_p})],
\end{aligned}
\end{equation*}
assuming $s\le s'$ and $t\le t'$ without loss of generality. The result follows if we show that $\hat F_\text{odd null}(t)\cip F_0(t)$ and $\hat F_\text{even null}(t)\cip F_0(t)$. This is so because
\begin{equation*}
\gamma_p\hat F_\text{odd null}(t)=2B_p-\hat F_\text{even}(t),
\end{equation*}
and $\hat F_\text{odd null}(t)\eqd\hat F_\text{even null}(t)$ by exchangeability.

Recall that
\begin{equation*}
\tau_p=\inf\{t>0:\frac{\#\{j:|\hat\beta_{2j-1}|-|\hat\beta_{2j}|\le-t\}/p}{\#\{j:|\hat\beta_{2j-1}|-|\hat\beta_{2j}|\ge t\}/p}\le q\},
\end{equation*}
which converges in probability to
\begin{equation*}
\tau_\text{KF}=\inf\{t>0:\frac{\gamma G_0(-t)+(1-\gamma)G_1(-t)}{\gamma (1-G_0(t))+(1-\gamma)(1-G_1(t))}\le q\},
\end{equation*}
according to the results we have, provided that $\tau_\text{KF}>0$. The condition $\tau_\text{KF}$ is satisfied if $q$ is small enough, and in practice we expect it to always hold (otherwise we would either reject all hypotheses or reject all the ones with non-zero $W_j$). The proof is exactly the same as Theorem~\ref{theorem:cutoff-converge}. The power then converges by Slusky's Theorem.

%Note that we only have to show convergence of CDFs for rational arguments, so we only use equation~\eqref{eq:lasso-amp-dist} countable times, which maintains the almost sure convergence.

\begin{figure}[H]
    \centering
\includegraphics[width = 0.9\textwidth]{figures/KF_lasso_power.pdf}
    \caption{Comparision of emprical and theoretical results of Knockoffs at FDR level $0.1$.} 
    \label{figure:comp_BH}
\end{figure}

==> discussion/representation.tex <==
\section{Models that admit a representation}
Let $X$ as a $p$-dimensional column vector admit representation $X=AU$, where $U$ is a $k$-dimensional column random vector, and $A$ is a $p\times k$ matrix. Suppose we are able to construct knockoff $\tilde U$ for $U$, e.g., it has independent elements. Let $B$ and $C$ be $p\times k$ matrices, and
\begin{equation}
\left(\begin{array}{c}
X\\
\tilde X
  \end{array}\right)=\left[
  \begin{array}{cc}
A & 0\\
B & C\\
  \end{array}
\right]\left(\begin{array}{c}
U\\
\tilde U
  \end{array}\right).
\end{equation}
Let $\GK_p=\{P\in\{0,1\}^{2p\times 2p}:P\text{ is a permutation matrix}, P_{ij}=0\text{ if }|i-j|\ne0\text{ or }p\}$. By definition, $\tilde X$ is knockoff of $X$ if and only if
\begin{equation}
P\left(\begin{array}{c}
X\\
\tilde X
  \end{array}\right)\sim\left(\begin{array}{c}
X\\
\tilde X
  \end{array}\right),\forall P\in\GK_p.
\end{equation}
A sufficient condition would thus be, for any $P\in\GK_p$, there exists a $Q\in\GK_k$, such that
\begin{equation}
P\left[
  \begin{array}{cc}
A & 0\\
B & C\\
  \end{array}
\right]=\left[
  \begin{array}{cc}
A & 0\\
B & C\\
  \end{array}
\right]Q,
\end{equation}
in which case
\begin{equation}
P\left(\begin{array}{c}
X\\
\tilde X
  \end{array}\right)=P\left[
  \begin{array}{cc}
A & 0\\
B & C\\
  \end{array}
\right]\left(\begin{array}{c}
U\\
\tilde U
  \end{array}\right)=\left[
  \begin{array}{cc}
A & 0\\
B & C\\
  \end{array}
\right]Q\left(\begin{array}{c}
U\\
\tilde U
  \end{array}\right)\sim\left[
  \begin{array}{cc}
A & 0\\
B & C\\
  \end{array}
\right]\left(\begin{array}{c}
U\\
\tilde U
  \end{array}\right)\sim\left(\begin{array}{c}
X\\
\tilde X
  \end{array}\right).
\end{equation}
In other words, if someone swaps the $i$th and $(i+p)$th rows of $\left[
  \begin{array}{cc}
A & 0\\
B & C\\
  \end{array}
\right]$, we can undo the effect by swapping its $j$th and $(j+k)$th columns, perhaps with multiple $j$'s.

It can be easily proved that if we have $A_{ij},A_{kj}\ne0$, $i\ne k$, then $B_{ij}=A_{ij}$ and $B_{kj}=A_{kj}$. Hence, there is one trivial optimal solution under these constraints.

The (almost) only way around this would be if the distribution is \emph{stable}, which means that if $X_1$ and $X_2$ are independent copies of $X$, then for any $a,b>0$, $aX_1+bX_2\sim cX+d$ for some constants $c>0$, $d\in\rr$. All stables distributions have been found, and a stable distribution is uniquely determined by four parameters through the characteristic function
\begin{equation}
\varphi(t;\alpha,\beta,c,\mu)=\exp(it\mu-|ct|^\alpha(1+i\beta\sign(t)\Phi)),\alpha\in(0,2],\beta\in[-1,1],c>0,\mu\in\rr,
\end{equation}
where
\begin{equation}
\Phi=\left\{
\begin{aligned}
&\tan(\frac{\pi\alpha}{2}),&\alpha\ne1\\
&-\frac2\pi\log|t|,&\alpha=1.
\end{aligned}
\right.
\end{equation}
The only special cases well known in statistical communities are the normal distribution ($\alpha=2$) and the Cauchy distribution ($\alpha=1$, $\beta=0$). They both happen to have multivariate generalizations as treatable elliptical distributions in Section \ref{sec:knockell}. Note that only the distribution with $\alpha=2$ (Gaussian) has finite second moment.
